Selective Sampling and Mixture Models in Generative Adversarial Networks

In this paper, we propose a multi-generator extension to the adversarial training framework, in which the objective of each generator is to represent a unique component of a target mixture distribution. In the training phase, the generators cooperate to represent, as a mixture, the target distribution while maintaining distinct manifolds. As opposed to traditional generative models, inference from a particular generator after training resembles selective sampling from a unique component in the target distribution. We demonstrate the feasibility of the proposed architecture both analytically and with basic Multi-Layer Perceptron (MLP) models trained on the MNIST dataset.

==> Selective Sampling and Mixture Models in Generative Adversarial Networks/chapters/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


We proposed a more detailed representation learning model based on a multi-generator extension to the GAN architecture. The generators tend to cooperatively resemble the target data distribution but each generator tends to produce only a distinct mode. This architecture provides selective sampling from a certain cluster of the target without the need of any labeling information.

==> Selective Sampling and Mixture Models in Generative Adversarial Networks/chapters/experiments-and-results.tex <==
\section{Experiments and results}
\label{sec:experiments-and-results}

\subsection{Experimental setup}
\label{subsec:experimental-setup}
We test and evaluate the proposed model on the MNIST dataset \cite{LeCun_1998_LeNet} and with the two-model case\footnote{We delegate the many model $K>2$ case to a future work. Our initial experiments show that the derived value function is unbalanced (i.e., divergences are unequally bounded and weighted) which results in degradation of the perceptual quality as the number of models increase.} $K=2$. In each test case, we select images from a two-digit combination (e.g, $\{0,\,1\}$) and train the randomly initialized model on the unlabeled dataset. We expect that each of the two generators will synthesize images of a unique digit. 

The latent random vector is uniformly distributed $\underline{z}\sim \mathcal{U}(\minus\,1, 1)$ in a 100-dimensional space $\underline{z}\in \mathbb{R}^{100}$ and it seeds two generators $g_1$ and $g_2$ where each is a 2-layer, feed-forward, fully connected neural network. Both the observed variable and the synthesized one belong to the same space $\underline{x},\hat{\underline{x}} \in \mathbb{R}^{784}$ and both are used to train the adversarial discriminator\footnote{A single binary discriminator for $g_1$ petted against $g_2$.} $h$. We use a single supplementary discriminator $h_1$ whose input is a batch of the synthesized images $\hat{\underline{x}}$. The two discriminators $h$ and $h_1$ are identically structured and have exactly the inverse architecture of the generators (except for the output layer). The output layer of each model uses logistic sigmoidal activation whereas its hidden layers use rectified linear units \cite{Nair_2010_ReLU_RBM}. The whole model is 4-layer deep in its longest path and comprises 0.8M trainable parameters. Finally, all models are trained using the Adam optimizer \cite{Kingma_2014_ADAM} with a learning rate of $10^{-3}$ and each sub-model gains a single parameter-update step in each iteration.

We highlight that instead of adhering to the aforementioned theoretical analysis in which training alternates between gradient-descent and -ascent steps, we rather flip the desired output $y\leftarrow 1-y$ and use only gradient-descent. This technique has been proposed in several previous works \cite{Goodfellow_2016_NIPSTutorial, Mao_2017_LSGAN} with conceivable reasoning\footnote{More recent studies proved that such an approach indeed eliminates the vanishing gradient problem but rather introduces critical sources of instability in the training process \cite{Arjovsky_2017_PrincipledMethods}.} but rather violates the presented analytical study of the architecture since each sub-model retains a different objective function.

\begin{figure}[t]
	\begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0}]
	\node (a) {\includegraphics[width=\linewidth, totalheight=0.13\linewidth]{./figures/DIGITS01_DIS0_EPOCH0002999_019.png}};
	\node (a) [below = 2mm of a.south, anchor=north] {\includegraphics[width=\linewidth, totalheight=0.13\linewidth]{./figures/DIGITS17_DIS0_EPOCH0002999_019.png}};
	\node (a) [below = 2mm of a.south, anchor=north] {\includegraphics[width=\linewidth, totalheight=0.13\linewidth]{./figures/DIGITS24_DIS0_EPOCH0002999_019.png}};
	\node (a) [below = 2mm of a.south, anchor=north] {\includegraphics[width=\linewidth, totalheight=0.13\linewidth]{./figures/DIGITS08_DIS1_EPOCH0002999_019.png}};
%	\node (a) [below = 2mm of a.south, anchor=north] {\includegraphics[width=\linewidth, totalheight=0.13\linewidth]{./figures/DIGITS49_DIS0_EPOCH0004999_019.png}};
	\node (a) [below = 2mm of a.south, anchor=north] {\includegraphics[width=\linewidth, totalheight=0.13\linewidth]{./figures/DIGITS26_DIS1_EPOCH0002999_019.png}};
	\end{tikzpicture}
	\caption{Two-digit experiments on the proposed architecture using the MNIST dataset. The top-most row of each experiment shows
		a sample of the real images whereas the two lower rows depict synthesized samples from each generator.}
	\label{fig:two-digit-success}
	\vspace{-2.5mm}
\end{figure}
\begin{figure}[!ht]
	\begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0}]
	\node (a) {\includegraphics[width=\linewidth, totalheight=0.13\linewidth]{./figures/DIGITS04_DIS1_EPOCH0002999_019.png}};
%	\node (a) [below = 2mm of a.south, anchor=north] {\includegraphics[width=\linewidth, totalheight=0.13\linewidth]{./figures/DIGITS12_DIS1_EPOCH0003399_019.png}};
	\node (a) [below = 2mm of a.south, anchor=north] {\includegraphics[width=\linewidth, totalheight=0.13\linewidth]{./figures/DIGITS19_DIS0_EPOCH0004999_019.png}};
%	\node (a) [below = 2mm of a.south, anchor=north] {\includegraphics[width=\linewidth, totalheight=0.13\linewidth]{./figures/DIGITS27_DIS0_EPOCH0009999_019.png}};
	\end{tikzpicture}
	\caption{Examples of failure cases.}
	\label{fig:two-digit-failure}
	\vspace{-2.5mm}
\end{figure}



\subsection{Results and discussion}
\label{subsec:dicussion}

Fig. \ref{fig:two-digit-success} shows the output of each generator in various experiments (each with a distinct two-digit combination). As observed, the generators produce samples of moderate to high perceptual quality but each one synthesizes a different digit from the given combination. On the other hand, few failure cases were observed and are shown in Fig. \ref{fig:two-digit-failure}. In these experiments, we still observe that the generators tend to produce, to some extent, different representations of the same digit rather than distinct digits.

Training adversarial networks, in general, is known to be unstable \cite{Arjovsky_2017_PrincipledMethods}, and the alternating gradient-based parameter updates (rather than training to completion) between the two sub-models in the original model is one of the sources for their instability \cite{Arjovsky_2017_PrincipledMethods}. In the proposed architecture, these alternating parameter updates are extended to a larger number of sub-models and, as a result, expected to amplify this instable training behavior. However, we observed in our experiments that the generators maintain distinct manifolds even in the early training steps and only collapse to the same digit when over-trained.

Furthermore, the objective of the supplementary discriminators is to provide a simple means for exploiting the powerful back-propagation algorithm in pushing the generators' distributions apart from each other. This seems to be valid as long as these models are weak classifiers. If they are provided with enough training capacity, they begin to deliver their discrimination task all by themselves and their driving force on the generators' distributions disappears. As a results, the generators tend to collapse to the same mode which is highly-rewarded by the adversarial discriminator rather than adhering to distinct classes. In fact, the precise amount of training, even for traditional GAN models, is a challenging hyper-parameter to optimize for reasons explained in \cite{Arjovsky_2017_PrincipledMethods}.



%However, we constrained our model to a naiive architecture and, therefore, observed some of these challenges. The unstable training behavior was also observed in the proposed architecture 
%
%Despite the recent progress in stabilizing and improving adversarial training, we limit this study to the very basic procedure in order to verify the feasibility of this approach. We expect that utilizing recent tricks in training GAN architecture (such as $\mathcal{L}_1$- and $\mathcal{L}_2$-loss \cite{Isola_2016_Pix2Pix, Apple, C2ycleConsistent}, batch normalization \cite{Radford_2015_DCGAN}, mini-batch discrimination \cite{Salimans_2016_ImprovedGAN}, penalizing confident decisions \cite{Salimans_2016_ImprovedGAN, Grosse_2016_AdversarialPerturbations}, leaky activations \cite{Radford_2015_DCGAN}, cycle-consistent loss \cite{Zhu_2017_CycleConsistentGAN}, instance and injected noise \cite{Kaaeonderby_2016_InstanceNoiseGAN, Salimans_2016_ImprovedGAN} among others) will improve the obtained results. This is also proved by our preliminary experiment which are outside the scope of this paper.


==> Selective Sampling and Mixture Models in Generative Adversarial Networks/chapters/introduction-and-related-work.tex <==
\section{Introduction and Related Work}
\label{sec:introduction-and-related-work}

One of the popular unsupervised learning methods is generative modeling, and in the recent years a promising architecture, referred to as \ul{G}enerative \ul{A}dversarial \ul{N}etworks (GAN) \cite{Goodfellow_2014_GAN}, has attracted a wide interest due to their impressive success in various applications domains, including text-to-image generation \cite{Reed_2016_Text2Image}, image-to-image translation \cite{Isola_2016_Pix2Pix}, multi- and super-resolution image synthesis \cite{Denton_2015_LaplacianPyramids}, video generation \cite{Vondrick_2016_GeneratingVideos}, in addition to a variety of  unsupervised and semi-supervised learning tasks \cite{Shrivastava_2016_SimulatedGANApple, Springenberg_2015_CatGAN, Zhu_2017_CycleConsistentGAN}. The common principle behind all variants of the GAN architecture is to exploit the discriminative power of neural networks in training generative counterparts. GAN models represent a compromise between ease of sampling and perceptual quality of synthesized samples.


Similar to other generative models, the ultimate objective of GANs is to model a target distribution from a limited set of observations.


% In addition, GANs feature ease of sampling with high perceptual quality \cite{}. 
% A generative network is tasked with estimating a real data distribution, while a discriminative one is tasked with training the former how to achieve their task. The generator does not explicitly model the real data distribution; instead, it learns how to synthesize data samples that are almost indistinguishable from the real ones.
% GANs resemble a compromise between ease of sampling and perceptual quality. When compared to Maximum Likelihood (ML) models, the latter tend to over-generalize the target distribution at the expense of perceptual quality \cite{Theis_2015_GANEvaluation}.

==> Selective Sampling and Mixture Models in Generative Adversarial Networks/chapters/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

%One of the popular unsupervised learning methods is generative modeling, and i

Over the last few years, a promising generative modeling architecture, referred to as \underline{G}enerative \underline{A}dversarial \underline{N}etwork (GAN) \cite{Goodfellow_2014_GAN}, has attracted a wide interest due to their impressive success in various application domains, including text-to-image generation \cite{Reed_2016_Text2Image}, compressive sensing \cite{Quan_2017_RefineGAN_CS_MRI}, image-to-image translation \cite{Isola_2016_Pix2Pix}, multi- and super-resolution image synthesis \cite{Denton_2015_LaplacianPyramids}, video generation \cite{Vondrick_2016_GeneratingVideos}, human driver modeling \cite{Kuefler_2017_GAIL_DriverGAN} in addition to a variety of  unsupervised and semi-supervised learning tasks \cite{Shrivastava_2016_SimulatedGANApple, Springenberg_2015_CatGAN, Zhu_2017_CycleConsistentGAN}. The common principle behind all variants of the GAN architecture is to exploit the discriminative power of neural networks in training generative counterparts. GAN models represent a compromise between ease of sampling and perceptual quality of synthesized samples.

Similar to other generative models, the ultimate objective of GANs is to model a target distribution from a limited set of observations. To this end, a basic GAN architecture consists of a cascade of two sub-models, a \emph{generator} $g$ whose objective is to synthesize samples $\hat{\underline{x}}$ indistinguishable from real observations $\underline{x}$, and a \emph{discriminator} $h$ whose objective is to train the generator by estimating a \emph{distance} between the generator's induced distribution $\mathbb{P}_{\hat{\underline{x}}}$ and the target one $\mathbb{P}_{{\underline{x}}}$. In spite of several difficulties in their training process, GAN models proved to be successful in synthesizing plausible, realistic samples while maintaining ease of sampling even for high-dimensional densities \cite{Arjovsky_2017_WassersteinGAN}. Consequently, extensive research has been carried out in order to understand and improve the training process of GAN models \cite{Salimans_2016_ImprovedGAN, Arjovsky_2017_PrincipledMethods, Arjovsky_2017_WassersteinGAN, Mao_2017_LSGAN, Yi_2017_DualGAN}, introduce this model to novel application domains \cite{Isola_2016_Pix2Pix, Zhu_2017_CycleConsistentGAN, Reed_2016_Text2Image, Zhu_2016_iGAN, Li_2016_TextureGAN}, and improve the basic formulation for more advanced learning tasks \cite{Springenberg_2015_CatGAN, Denton_2015_LaplacianPyramids, Wang_2016_S2GAN, Mirza_2014_cGAN, Makhzani_2015_AdversarialAE}.

In this paper, we propose an extension to the basic GAN architecture that targets a more detailed representation of the real data manifold. More specifically, in the proposed architecture, multiple generators cooperate in resembling a target data distribution while maintaining distinct manifolds. All generators are trained using a single adversarial discriminator but are also constrained to distinct distributions via a set of supplementary discriminators. The ultimate objective of the architecture is a set of generative functions learned from a finite set of data samples that jointly model the target data distribution but individually resemble distinct modes in it.



% In addition, GANs feature ease of sampling with high perceptual quality \cite{}. 
% A generative network is tasked with estimating a real data distribution, while a discriminative one is tasked with training the former how to achieve their task. The generator does not explicitly model the real data distribution; instead, it learns how to synthesize data samples that are almost indistinguishable from the real ones.
% GANs resemble a compromise between ease of sampling and perceptual quality. When compared to Maximum Likelihood (ML) models, the latter tend to over-generalize the target distribution at the expense of perceptual quality \cite{Theis_2015_GANEvaluation}.

==> Selective Sampling and Mixture Models in Generative Adversarial Networks/chapters/model-architecture.tex <==
\section{Model Architecture}
\label{sec:model-architecture}

Let $\underline{x} \in \mathcal{X}$ be the observed data of a continuous random vector $\underline{x}$ from the space $\mathcal{X}$ of observations. The notation $\underline{x} \sim p_{\underline{x}}$ is used to denote the probability density function (pdf) $p_{\underline{x}}$ of $\underline{x}$ of the real data distribution $\mathbb{P}_{\underline{x}}$.

The proposed architecture is depicted in Fig. \ref{fig:model-architecture} and consists of $K$ generative models (generators) $\{g_k\}_{k=1}^{K}$, each of which maps a latent variable $\underline{z}_k\sim p_{\underline{z}}$ to a synthesized sample $\smash{\hat{\underline{x}}_k = g_k(\underline{z}_k)}\sim p_k$ and induces a continuous\footnote{For simplicity, and for illustrative purposes, we shall assume that all distributions are continuous with non-disjoint support.} distribution $\mathbb{P}_k$. All synthesized samples $\hat{\underline{x}}_k$ belong to the same space $\mathcal{X}$. Let $p_{\underline{x}}$ be the density function of the real data distribution $\smash{\mathbb{P}}_{\underline{x}}$. Furthermore, let $\hat{\underline{x}}$ be a random vector equi-probably sampled from $\{g_k\}_{k=1}^{K}$. This results in a mixture pdf $p_{\hat{\underline{x}}}$ defined as
\begin{equation}
p_{\hat{\underline{x}}}(\underline{x}) =\; \frac{1}{K} \sum_{k=1}^K p_k(\underline{x})
\label{eq:mixture-model}
\end{equation}%
We further introduce $K$ binary logistic models (discriminators) $\{h_k\}_{k=1}^{K}$ each of which maps samples from the input data space $\hat{\underline{x}}\sim\mathcal{X}$ to a probability $h_k: \mathcal{X} \rightarrow [0, 1]$ where $h_k(\hat{\underline{x}})$ resembles the probability that $\hat{\underline{x}}$ is sampled from the $k^\text{th}$ model $g_k$ as opposed to all other components in the mixture. The opposite probability that $\hat{\underline{x}}$ is equi-probably sampled from the remaining set of generators $g_j,\,j\neq k$ is
\begin{equation}
p_{\bar{k}}(\underline{x}) = \frac{1}{K-1} \sum_{\substack{j=1\\j\neq k}}^{K} p_j(\underline{x})
\end{equation}
which also gives another formulation for the mixture pdf
\begin{equation}
p_{\hat{\underline{x}}}(\underline{x}) =\; \frac{1}{K} \sum_{k=1}^K p_{\bar{k}}(\underline{x})
\label{eq:complement-mixture-model}
\end{equation}
The loss function of each of the $k^\text{th}$ discriminator becomes
{\small
\begin{align*}
\mathcal{L}_{h_k}  
& =                                    \mathbb{E}_{\underline{z} \sim p_{\underline{z}}         }             \log\left(     h_k(g_k(\underline{z})) \right) + 
    \sum_{\substack{j=1\\j\neq k}}^{K} \mathbb{E}_{\underline{z} \sim p_{\underline{z}}         }             \log\left( 1 - h_k(g_j(\underline{z})) \right) \\
& =                                    \mathbb{E}_{\underline{x} \sim p_k         }             \log\left(     h_k(    \underline{x})  \right) + 
    \sum_{\substack{j=1\\j\neq k}}^{K} \mathbb{E}_{\underline{x} \sim p_j         }             \log\left( 1 - h_k(    \underline{x})  \right) \\
& =                                    \mathbb{E}_{\underline{x} \sim p_k         }             \log\left(     h_k(    \underline{x})  \right) + 
                                       \mathbb{E}_{\underline{x} \sim p_{\bar{k}} } \left[(K-1) \log\left( 1 - h_k(    \underline{x})  \right) \right] \\
\end{align*}}%






Moreover, an additional adversarial discriminator $h$ distinguishes samples of the real mixture distribution $\mathbb{P}_{\underline{x}}$ from those of the generators' mixture $\mathbb{P}_{\hat{\underline{x}}}$. The loss function of this discriminator is similar to the traditional GAN loss 
{\small \begin{align*}
	\mathcal{L}_{h}  
	& =\mathbb{E}_{\underline{x} \sim p_{     \underline{x}}}\log\left(     h(\underline{x}) \right) + 
	\mathbb{E}_{\underline{x} \sim p_{\hat{\underline{x}}}}\log\left( 1 - h(\underline{x}) \right) \\
	\end{align*}}%




Let $V$ be the value function of the \emph{mini-minimax} game defined as
{\small \begin{align}
	\min_{\{g_k\}} \min_{\{h_k\}} \max_{h} V = \mathcal{L}_{h} - \sum_{k=1}^{K} \mathcal{L}_{h_k} 
	%\min_{g_1, ..., g_K} \min_{h_1, ..., h_K} \max_{h} V = \mathcal{L}_{h} - \sum_{k=1}^{K} \mathcal{L}_{h_k} \\
	\end{align}}%
The adversarial GAN game in this case becomes a \emph{minimax} game between two teams. The first team consists of a single player (the adversarial discriminator $h$) whose objective is to \emph{maximize} the value function. The second team consists of all generators $\{g_k\}_{k=1}^{K}$ and supplementary discriminators $\{h_k\}_{k=1}^{K}$ where each player in this team is tasked with \emph{minimizing} the same value function. Each model optimizes the value function with respect to its own parameters (assuming all other models are fixed).


In the non-parametric limit, and assuming each model can train to completion, the resulting discriminators reach their global optimum at (proof can be found in \cite{Goodfellow_2014_GAN})
{\small \begin{equation*}
h_k^\star(\underline{x}) =\, \frac{p_k(\underline{x})}{p_k(\underline{x}) + (K-1) \cdot p_{\bar{k}}(\underline{x})} =\, \frac{p_k(\underline{x})}{K \cdot p_{\hat{\underline{x}}}(\underline{x})}
\end{equation*}}%
and
{\small \begin{equation*}
h^\star(\underline{x})   =\, \frac{p_{{\underline{x}}}(\underline{x})}{p_{\hat{\underline{x}}}(\underline{x})\; +\; p_{{\underline{x}}}(\underline{x})}
\end{equation*}}%
Substituting these optimal values in the value function $V$ results in 
{\small \begin{alignat*}{3}
V && =\; &&&                       \mathbb{E}_{\underline{x} \sim p_{\underline{x}}      }        \log\left(     h^\star  (\underline{x}) \right) 
           +                       \mathbb{E}_{\underline{x} \sim p_{\hat{\underline{x}}}}        \log\left( 1 - h^\star  (\underline{x}) \right)  \\
  && -\; &&& \sum_{k=1}^{K} \left( \mathbb{E}_{\underline{x} \sim p_k                    }        \log\left(     h_k^\star(\underline{x}) \right) +
                                   \mathbb{E}_{\underline{x} \sim p_{\bar{k}}            }        \log\left( 1 - h_k^\star(\underline{x}) \right) \right) \\
  && =\; &&&                       \mathbb{E}_{\underline{x} \sim p_{\underline{x}}      }        \log\left(\frac{p_{{\underline{x}}}(\underline{x})}{p_{\hat{\underline{x}}}(\underline{x})\; +\; p_{{\underline{x}}}(\underline{x})}     \right) \\ 
  && +\; &&&                       \mathbb{E}_{\underline{x} \sim p_{\hat{\underline{x}}}}        \log\left(\frac{p_{\hat{\underline{x}}}(\underline{x})}{p_{\hat{\underline{x}}}(\underline{x})\; +\; p_{{\underline{x}}}(\underline{x})} \right) \\
  && -\; &&& \sum_{k=1}^{K}        \mathbb{E}_{\underline{x} \sim p_k                    }  \left[\log\left(\frac{p_k                    (\underline{x})}{p_{\hat{\underline{x}}}(\underline{x})}  \right) + \log\left(\frac{1}{K}\right)                      \right] \\
  && -\; &&& \sum_{k=1}^{K}        \mathbb{E}_{\underline{x} \sim p_{\bar{k}}            }  \left[\log\left(\frac{p_{\bar{k}            } (\underline{x})}{p_{\hat{\underline{x}}}(\underline{x})} \right) + \log\left(\frac{K-1}{K}\right)                    \right] \\
\end{alignat*}\vspace{-10mm}}%

All terms in the previous equation resemble different, non-symmetric Kullback-Leibler (KL) divergences resulting in 
{\small \begin{alignat}{3}
V && =\; &&&                \KLD \left( \mathbb{P}_{\underline{x}}        \;\|\;  \mathbb{P}_{\hat{\underline{x}}} \plus\; \mathbb{P}_{{\underline{x}}}    \right) + 
                            \KLD \left( \mathbb{P}_{\hat{\underline{x}}}  \;\|\;  \mathbb{P}_{\hat{\underline{x}}} \plus\; \mathbb{P}_{{\underline{x}}}    \right) \nonumber \\ 
  && -\; &&& \sum_{k=1}^{K} \KLD \left( \mathbb{P}_k                      \;\|\;  \mathbb{P}_{\hat{\underline{x}}}                                         \right) - 
             \sum_{k=1}^{K} \KLD \left( \mathbb{P}_{\bar{k}}              \;\|\;  \mathbb{P}_{\hat{\underline{x}}}                                         \right) \nonumber \\
  && -\; &&& K\cdot\log\left(\frac{K-1}{K^2}\right) 
\label{eq:generator-value-function-kl}
\end{alignat}}%
It can be further simplified to symmetric Jensen-Shannon (JS) divergences
{\small \begin{alignat}{3}
V  && =\; &&& 2\cdot\JSD \left( \mathbb{P}_{\hat{\underline{x}}},  \mathbb{P}_{{\underline{x}}}   \right) \nonumber - K\cdot \JSD \left( \mathbb{P}_{{1}}, \dots, \mathbb{P}_{{K}}  \right) \nonumber \\
   && -\; &&&  K\cdot\JSD \left( \mathbb{P}_{\bar{1}}, \dots, \mathbb{P}_{\bar{K}} \right) - K\cdot\log\frac{K-1}{K^2} - \log 4
\label{eq:generator-value-function}
\end{alignat}}%
where the $\pi$-generalized JS divergence for a finite mixture of distributions is defined as \cite{Lin_1991_ShannonDivergences}
%{\small \begin{alignat*}{3}
%   \JSD(\mathbb{P}_{1}, \dots, \mathbb{P}_K)   =\;\frac{1}{K}\sum_{k=1}^{K}\KLD\left(\mathbb{P}_k\;\Big\|\;\frac{1}{K}\sum_{j=1}^{K}\mathbb{P}_j\right)
%\end{alignat*}}%
{\small \begin{equation}
    \JSD^{\pi_1, \dots, \pi_K}(\mathbb{P}_{1}, \dots, \mathbb{P}_K) =\; \sum_{k=1}^{K}\pi_k\cdot\KLD\left(\mathbb{P}_k\;\Big\|\;\sum_{j=1}^{K}\pi_j\cdot\mathbb{P}_j\right)
    \label{eq:jensen-shannon-mixture}
\end{equation}}%
where $\pi_1,\dots,\pi_K$ are the distributions' weights and are assumed in this work to be $1/K$. Eq. \ref{eq:jensen-shannon-mixture} is applicable to the two distributions $\mathbb{P}_{{\underline{x}}}$ and $\mathbb{P}_{\hat{\underline{x}}}$ by defining an average distribution $\mathbb{P}_A = (\mathbb{P}_{\hat{\underline{x}}} + \mathbb{P}_{{\underline{x}}}) / 2$. It is also applicable within the mixture model $\mathbb{P}_{\hat{\underline{x}}}$ using Eq. \ref{eq:mixture-model} and \ref{eq:complement-mixture-model}.
Minimizing Eq. \ref{eq:generator-value-function} is equivalent to minimizing the \emph{difference} between the real data distribution and the estimated one while maximizing the dissimilarity between the components of the latter. This, in turn, induces each generator in the model to maintain distinct observational claims of the real data distribution. 


\begin{figure}[!t]
	\input{./figures/model-architecture.tex}
	\vspace{-5.0mm}
\end{figure}

Eq. \ref{eq:generator-value-function-kl} represents a very interesting objective function. The first two terms resemble the symmetric JS divergence between the real distribution and the estimated mixture which is non-negative and retains its minimum when $\mathbb{P}_{\underline{x}} = \mathbb{P}_{\hat{\underline{x}}}$. This term is the common measure in traditional GAN models \cite{Goodfellow_2014_GAN}. The third KL-divergence prevents any of the component models $g_k$ from prevalence (representing the whole mixture all by itself), whereas the last term prevents the same component from vanishing. 

In practice, each model (either a discriminator or a generator) is a parametric Multi-Layer Perceptron (MLP). This, of course, limits the family of density functions representable by each generator. Nevertheless, each one retains its own parameters, and as a result, the estimated distribution represents a heterogeneous mixture model. Training is straightforward and, similar to traditional GANs, consists of alternating gradient-based parameter updates. Gradient-ascent is utilized by the adversarial discriminator while the supplementary discriminators and the generators use gradient-descent.



==> Selective Sampling and Mixture Models in Generative Adversarial Networks/chapters/related-work.tex <==
\section{Related work}
\label{sec:realted-work}

The original architecture of a GAN model consisted of a single generator, whose objective is to synthesize data samples that are indistinguishable from real ones, and an adversarial discriminator, which attempts to distinguish between real data samples and generated ones \cite{Goodfellow_2014_GAN, Goodfellow_2016_NIPSTutorial}. Both models are trained simultaneously and in an adversary. When successfully trained, the generator tends to synthesize realistic samples, whereas the discriminator is expected to become maximally confused. Sampling in this architecture consists of sampling a latent variable from a simple distribution (e.g., standard Gaussian) and mapping its value to the sample space using the generator's function. Despite the simplicity of such a process, it is unrestrained over the whole target data manifold. In other words, there is no control on the samples being synthesized by the generator.

In \cite{Radford_2015_DCGAN}, it was observed that the generator tends to structure the latent space, and the complex transformations in the sample space (e.g., face pose) can be controlled via a simple linear interpolation on the latent variable. This feature was exploited in \cite{Chen_2016_InfoGAN} by discretizing a subset of the latent variable attributes in order to control the sampling process. This approach, however, limits the trained generator to a single estimation of the density function whose output can be controlled by conditioning on the selected attributes. In a like manner, Conditional GANs (cGAN) \cite{Mirza_2014_cGAN, Sricharan_2017_SScGAN} controlled this sampling process by conditioning the generator on an observed variable in addition to the latent one. Examples of conditioning variables include text embeddings \cite{Reed_2016_Text2Image}, foreign domain image \cite{Isola_2016_Pix2Pix, Denton_2015_LaplacianPyramids}, or class attributes \cite{Mirza_2014_cGAN}. However, cGAN models require the additional information found in the conditioning variable and are incapable of learning hidden structures of the target distribution in an unsupervised fashion. 

Coupled GAN models \cite{Liu_2016_CoGAN} introduced a multi-generator multi-discriminator architecture whose objective is to learn the joint distribution of multi-domain images from their marginal ones. For a given realization of the latent variable, each generator synthesizes the same sample but in different domains. While this approach eliminates the need for inter-domain knowledge, it requires the complete knowledge of each domain in advance.

Categorical GANs \cite{Springenberg_2015_CatGAN} resemble one of the promising approaches to unravel hidden structures in unlabeled data manifolds. The binary logistic discriminator in traditional GAN models is replaced by a multi-class one whose objective is to maintain high confidence classification scores for the real data samples while being maximally uncertain when provided with synthesized images. As a result, the discriminator becomes capable of clustering the real data samples in a completely unsupervised fashion. Nevertheless, this approach adopts a single generator which is still uncontrolled in its sampling process.

Our approach differs in that its objective is the controlled generation process rather than discrimination. The proposed GAN model attempts to control the sampling process by training several generators that collectively resemble the targeted distribution while maintaining distinct modes among these generators. One can selectively sample from a certain sub-population by sampling from the corresponding generator only. 

%The seed to the generator is a latent variable from a known probability distribution. Common approaches use a multivariate Gaussian or uniform distributions \cite{Goodfellow_2014_GAN} but seeding the generator with a more informative variable (such as synthetic data as in \cite{Shrivastava_2016_SimulatedGANApple}) is also possible. GANs were also proposed in a conditional setting in which the generator, and optionally the discriminator, is conditioned on an observed variable in addition to the latent one in order to guide the synthesis process. 

%In this paper, we propose an extension to the basic framework whose objective is to capture more fine-grained representation of the real data distribution in an unsupervised setting. Our architecture differs from previous work in that it estimates the component densities of a mixture of $N$-subpopulations from the \emph{empirical} marginal density, resulting in both generative models capable of estimating a unique sub-population in the target signal, and discriminative models capable of clustering (distinguishing) samples coming from such populations.
%
%The set of trained \emph{generators} in an out architecture represent $N$-heterogeneous components whose mixture build up an estimate of the marginal distribution of the observed variable. Sampling from a generator is trivial (as it corresponds to a single feed-forward inference pass of an MLP) and resembles drawing samples from a certain sub-population of $p_\text{data}$. The mixture model is only limited by the space of density function representable by the generator model, and since each generator retains its own parameters, the mixture can have a set of heterogeneous models. 

%CatGAN \cite{Springenberg_2015_CatGAN}

% Several variants of this basic architecture have been proposed with the common objective of either stabilizing the training process or guiding the generative 
% Energy-based models were introduced into the GAN architecture to replace the traditional logistic binary classifier primarily used in the discriminator \cite{Zhao_2016_EBGAN}. Energy-based GAN models are expected to maintain more stable training behavior.

%Additionally, multiple GAN architectures are applied in a hierarchical architecture (essentially a combination of unconditional and conditional GANs) \cite{Wang_2016_S2GAN} which is advantageous in learning a multi-stage representation.

% A major problem in GAN training is the stochasticity of the generated samples. Several previous works have observed that the generator can collapse to a deterministic output that retains minimal gradients from the discriminator. Regularization terms were introduced to encourage stochasticity in the generator's output such as mini-batch discrimination \cite{Salimans_2016_ImprovedGAN}, pull-away term \cite{Zhao_2016_EBGAN}, or maintaining stochastic layers (such as DropOut) during the inference phase \cite{Isola_2016_Pix2Pix}.






%From an architectural prospective, this work represents a breadth expansion of the basic two-player GAN game where multiple generators and discriminators are simultaneously trained. GAN variants that contain multiple, simultaneously trained models were also proposed in several previous works. For example, two-way inverse GAN models were proposed in \cite{Zhu_2017_CycleConsistentGAN} for unsupervised image-to-image translation. In \cite{Denton_2015_LaplacianPyramids}, a sequel of GANs was able to synthesis plausible high-resolution images in a coarse-to-fine fashion. The .... nature of imagery data was exploited in \cite{S2-GAN} with two separate models; one building the spatial structure while the other stylize the generated scene. Similarly, a two-stream GAN architecture that model a scene's foreground separately from its background is proposed in \cite{Vondrick_2016_GeneratingVideos} for video generation.
%
%
%Applications of this approach include selective sampling, mixture analysis, and deep unsupervised clustering. The main target is a set of generator each is capable of synthesizing images from a unique subset of the real data. In theory, we expect this architecture to better represent a heterogeneous mixture of densities if the generators' model has enough capacity to estimate each component density. Moreover, and as an auxiliary output, supplementary models are trained to distinguish between synthesized images on a per-generator basis. As a result, these discriminator models become capable of clustering current and future data samples as long as they are identically distributed.





==> Selective Sampling and Mixture Models in Generative Adversarial Networks/figures/cnn_net.tex <==
%draw a cnn layer with input and output feature maps and with kernels
\scalebox{0.5}{
\begin{tikzpicture}
    \definecolor{myblue}{cmyk}{1,0,0,0}
    \definecolor{myred}{cmyk}{0,1,0,0}
    \node[] at (0.5,5.5,0) {\Large \bf The convolutional layer};
    
    %draw input feature map
    \draw[white](0,0,0)--(0,4,0)--(1,4,0)--(1,0,0)--(0,0,0);
    \draw[white](1,0,0)--node[color=black,right]{$M$}(1,0,4)--(1,4,4)--(1,4,0)--(1,0,0);
    \draw[white](1,0,4)--node[color=black,below]{$O$}(0,0,4)--(0,4,4)--(1,4,4)--(1,0,4);
    \draw[white](0,0,4)--(0,0,0)--(0,4,0)--(0,4,4)--node[color=black,left]{$N$}(0,0,4);
    %caption
    \node[] at (0.5,4.5,0) {Input $\X$};
                
    %draw first kernel
    \draw[white](3.5,0.5,1.5)--(3.5,1.5,1.5)--(4.5,1.5,1.5)--(4.5,0.5,1.5)--(3.5,0.5,1.5);
    \draw[white](4.5,0.5,1.5)--(4.5,0.5,2.5)--(4.5,1.5,2.5)--(4.5,1.5,1.5)--(4.5,0.5,1.5);
    \draw[white](4.5,0.5,2.5)--(3.5,0.5,2.5)--(3.5,1.5,2.5)--(4.5,1.5,2.5)--(4.5,0.5,2.5);
    \draw[white](3.5,0.5,2.5)--(3.5,0.5,1.5)--(3.5,1.5,1.5)--(3.5,1.5,2.5)--(3.5,0.5,2.5);
    
    %draw dots inbetween
    \draw[dashed](3.5,1.5,1.5)--(3.5,2.5,1.5);
    \draw[dashed](4.5,1.5,1.5)--(4.5,2.5,1.5);
    \draw[dashed](4.5,1.5,2.5)--(4.5,2.5,2.5);
    \draw[dashed](3.5,1.5,2.5)--(3.5,2.5,2.5);
    
    %draw second kernel
    \draw[white](3.5,2.5,1.5)--(3.5,3.5,1.5)--(4.5,3.5,1.5)--(4.5,2.5,1.5)--(3.5,2.5,1.5);
    \draw[white](4.5,2.5,1.5)--(4.5,2.5,2.5)--(4.5,3.5,2.5)--(4.5,3.5,1.5)--(4.5,2.5,1.5);
    \draw[white](4.5,2.5,2.5)--node[color=black,below]{$\:\:O$}(3.5,2.5,2.5)--(3.5,3.5,2.5)--(4.5,3.5,2.5)--(4.5,2.5,2.5);
    \draw[white](3.5,2.5,2.5)--(3.5,2.5,1.5)--(3.5,3.5,1.5)--node[color=black,left]{$K$}(3.5,3.5,2.5)--node[color=black,left]{$K$}(3.5,2.5,2.5);
    %caption
    \node[] at (3.5,3.5,0) {Kernel tensor $\W$};
    
    %draw input feature maps
    \foreach \x in {0,0.25,0.5,0.75,1}{    
        \pgfmathsetmacro\k{(\x+0.1)*50}
            \draw[black, fill=black!\k](\x,0,4)--(\x,0,0)--(\x,4,0)--(\x,4,4)--(\x,0,4);}
    
    %draw selected region for convolution
    \draw[black](1,2,3)--(1,2,2)--node[color=black,right]{$\X(m,n)$}(1,3,2)--(1,3,3)--(1,2,3);
    
    %draw connections to kernels
    \draw[dashed](1,2,3)--(3.5,0.5,2.5);
    \draw[dashed](1,3,3)--(3.5,3.5,2.5);
    \draw[dashed](1,2,2)--(3.5,0.5,1.5);
    \draw[dashed](1,3,2)--(3.5,3.5,1.5);
    
    %draw first kernel
    \foreach \x in {0,0.25,0.5,0.75,1}{    
        \pgfmathsetmacro\k{(\x+0.1)*100}
        \draw[black, fill=myblue!\k](3.5+\x,0.5,2.5)--(3.5+\x,0.5,1.5)--(3.5+\x,1.5,1.5)--(3.5+\x,1.5,2.5)--(3.5+\x,0.5,2.5);}

    %draw second kernel
    \foreach \x in {0,0.25,0.5,0.75,1}{    
        \pgfmathsetmacro\k{(\x+0.1)*100}
        \draw[black, fill=myred!\k](3.5+\x,2.5,2.5)--(3.5+\x,2.5,1.5)--(3.5+\x,3.5,1.5)--(3.5+\x,3.5,2.5)--(3.5+\x,2.5,2.5);}
    
    %draw output feature map with convolution results
    \draw[black](7,0,0)--(7,4,0)--(8,4,0)--(8,0,0)--(7,0,0);
    \draw[black](8,0,0)--node[color=black,right]{$M-K+1$}(8,0,4)--(8,4,4)--(8,4,0)--(8,0,0);
    \draw[black](7,0,4)--(7,0,0)--(7,4,0)--(7,4,4)--node[right]{$N-K+1$}(7,0,4);
    
    \foreach \x in {0,0.25,0.5,0.75,1}{    
        \pgfmathsetmacro\k{(\x+0.1)*50}
        (1,2,3)--(1,2,2)--(1,3,2)--(1,3,3)--(1,2,3)
            \draw[black, fill=black!\k](\x+7,2.25,2.75)--(\x+7,2.25,2.25)--(\x+7,2.75,2.25)--(\x+7,2.75,2.75)--(\x+7,2.25,2.75);}
            
    \draw[black](8,0,4)--node[below]{$P$}(7,0,4)--(7,4,4)--(8,4,4)--(8,0,4);
    
    %draw connections to kernels
    
    \draw[dashed](4.5,3.5,2.5)--(7,2.75,2.75);
    \draw[dashed](4.5,0.5,1.5)--(7,2.25,2.25);
    \draw[dashed](4.5,3.5,1.5)--(7,2.75,2.25);
    
    %draw bias
    \foreach \y in {1,2,3,4,5}{    
        \pgfmathsetmacro\k{((\y-1)/4+0.1)*50}
            \fill [black!\k] (5 ,1-\y*0.5,2) rectangle (5.5,1.5-\y*0.5,2);}
    
    \draw[dashed](4.5,0.5,2.5)--(7,2.25,2.75);
    
    
    %caption
    \node[] at (7.5,4.5,0) {Activation $\A$};  
    \node[] at (4.5,-2.5,0) {Bias $\bi$};  
    
    %operators
    \node[] at (2.5,2,2) {$*$}; 
    \node[] at (5.25,2,2) {$+$};
    \node[] at (6.25,2,2) {$=$}; 
    
    %kernel index
    \node[] at (4,3,2) {$1$};
    \node[] at (4,1,2) {$P$}; 
    
    \draw[dashed](9.5,5,0)--(9.5,-2,0);
    \node[] at (9.5,-2.25,0) {unfolding};
    

    %draw unfolded 
    \node[] at (2.0+11-0.75,5.5,0) {\Large \bf The equivalent dense layer};
    \definecolor{myblue}{cmyk}{1,0,0,0}
    \definecolor{myred}{cmyk}{0,1,0,0}

    %captions
    \node[] at (1.5+10-0.75,5-0.5,0) {Activation $\ai$};
    \node[] at (1.5+10+3,5-0.5,0) {Kernel matrix $\Wu$};
    \node[] at (1.5+10+8,5-0.5,0) {Input $\x$};
    \node[] at (1.5+10+9.75,5-0.5,0) {Bias $\bi$};
    
    %operators
    \node[] at (1.5+10+0.5,2.75-0.5,0) {$=$};
    \node[] at (1.5+10+7.5,2.75-0.5,0) {$\cdot$};
    \node[] at (1.5+10+9.0,2.75-0.5,0) {$+$};
    
    %The unfolded matrix
    \foreach \x in {1,2,3,4,5}{
        \foreach \y in {1,2,3,4,5}{
            \pgfmathsetmacro\c{1.0-(\y-1)*0.25}
            \pgfmathsetmacro\m{(\y-1)*0.25}
            \definecolor{mix}{cmyk}{\c,\m,0,0}
            \pgfmathsetmacro\k{((\x-1)/5+0.1)*100}
            \fill [mix!\k] (1.5+10+2+\x*1,\y*0.5+1.5-0.5,0) rectangle (1.5+10+2+\x*1-1,\y*0.5-0.5+1.5-0.5,0);
         }
    }
    
    %draw unfolded input feature map
    \foreach \y in {1,2,3,4,5}{    
        \pgfmathsetmacro\k{((\y-1)/4+0.1)*50}
            \fill [black!\k] (1.5+10+8,4-\y-0.5,0) rectangle (1.5+10+8.5,4-\y+1-0.5,0);}
    
    %draw unfolded output feature map
    \foreach \y in {1,2,3,4,5}{    
        \pgfmathsetmacro\k{((\y-1)/4+0.1)*50}
            \fill [black!\k] (1.5+10-1,4-\y*0.5-0.5,0) rectangle (1.5+10-0.5,4.5-\y*0.5-0.5,0);}
    
    %draw bias
    \foreach \y in {1,2,3,4,5}{    
        \pgfmathsetmacro\k{((\y-1)/4+0.1)*50}
            \fill [black!\k] (1.5+10+9.5,4-\y*0.5-0.5,0) rectangle (1.5+10+10,4.5-\y*0.5-0.5,0);}
    
    %give the size of the unfolded matrix
    \node[] at (1.5+10+1.8,2.75-0.5,0) {$P$};
    \node[] at (1.5+8.8,2.75-0.5,0) {$P$};
    \node[] at (1.75+20,2.75-0.5,0) {$P$};
    \node[] at (1.5+10+4.5,4.2-0.5,0) {$K^2O$};
    \node[] at (1.5+10+9,1.5-0.5,0) {$K^2O$};
\end{tikzpicture}}


==> Selective Sampling and Mixture Models in Generative Adversarial Networks/figures/model-architecture.tex <==

\centering
%    \tikzset{trapezium stretches body=true}
\def\zgsep{7.5mm}
\def\gdsep{40mm}
\def\dssep{12.5mm}
\def\ysepa{14mm}
\def\ysepb{7.5mm}
\def\trpw{7.0mm}
\def\trph{7.0mm}
\def\tang{60}
\begin{tikzpicture}[every node/.style={inner sep=0.1mm,outer sep=0mm, font=\footnotesize},
generator/.style={anchor=north,      trapezium, trapezium angle=\tang, minimum width=\trpw, minimum height=\trph, rotate=90, rounded corners=1pt,  fill=SkyBlue1},
suppdiscr/.style={anchor=south west, trapezium, trapezium angle=\tang, minimum width=\trpw, minimum height=\trph, rotate=270, rounded corners=1pt, fill=Wheat2    },
score/.style={draw=none, anchor=center, outer sep=1mm},
latent/.style={draw=none, anchor=center, outer sep=1mm}]
\node (z1) [latent]                          {$\underline{z}_1$}; 
\node (z2) [latent, below=\ysepa of z1.center] {$\underline{z}_2$}; 
\node (z3) [latent, below=\ysepb of z2.center] {\large  $\cvdots$}; 
\node (z4) [latent, below=\ysepb of z3.center] {$\underline{z}_K$}; 

\node (g1) at ($(z1.center) + (\zgsep, 0mm)$) [generator, fill=SkyBlue1] { }; 
\node (g2) at ($(z2.center) + (\zgsep, 0mm)$) [generator, fill=SkyBlue2] { }; 
\node (g3) at (z3.center -| g2.center) [] {\large  $\cvdots$};  
\node (g4) at ($(z4.center) + (\zgsep, 0mm)$) [generator, fill=SkyBlue3] { }; 

\node (d1) at ($(g1.center) + (\gdsep, 0mm)$) [suppdiscr] { };  
\node (d2) at ($(g2.center) + (\gdsep, 0mm)$) [suppdiscr] { };        
\node (d4) at ($(g4.center) + (\gdsep, 0mm)$) [suppdiscr] { };  
\node (d3) at ($(d2.center)!0.5!(d4.center)$) [] {\large  $\cvdots$};         
\node (d0) at ($(d1.south west) + (0mm, 17mm)$) [suppdiscr, fill=Orchid1] {};         

\node (s0) at ($(d0.center) + (\dssep, 0mm)$) [score] {${s}$};
\node (s1) at ($(d1.center) + (\dssep, 0mm)$) [score] {${s}_1$};
\node (s2) at ($(d2.center) + (\dssep, 0mm)$) [score] {${s}_2$};
\node (s3) at (d3.center -| s2.center)       {\large  $\cvdots$};
\node (s4) at ($(d4.center) + (\dssep, 0mm)$) [score] {${s}_K$};

\node at (g1.center) {$g_1$}; 
\node at (g2.center) {$g_2$}; 
\node at (g4.center) {$g_K$}; 

\node at (d0.center) {$h$}; 
\node at (d1.center) {$h_1$}; 
\node at (d2.center) {$h_2$}; 
\node at (d4.center) {$h_K$}; 

\node (g0) at (g1.north |- d0.south west) [anchor=center, cylinder, shape border rotate=90, inner sep=1mm, minimum height=10mm, minimum width=10mm, fill=DarkSeaGreen3, draw=Green4] {};
\node at (g0.center) [anchor=center] {$\mathbb{P}_{\underline{x}}$};

\draw [arrows={ - Stealth[round]}, thick, DarkSeaGreen3] (g0.east) -- (d0.south west) 
node [pos=0.17, above=0.35mm, black] {$\underline{x}$} 
node [pos=0.83, above=0.35mm, black] {real};

\draw [arrows={ - Stealth[round]}] (d0.north) -- (s0.west);        
\draw [arrows={ - Stealth[round]}] (z1.east) -- (g1.north); \draw [arrows={ - Stealth[round]}] (d1.north) -- (s1.west);        
\draw [arrows={ - Stealth[round]}] (z2.east) -- (g2.north); \draw [arrows={ - Stealth[round]}] (d2.north) -- (s2.west);        
\draw [arrows={ - Stealth[round]}] (z4.east) -- (g4.north); \draw [arrows={ - Stealth[round]}] (d4.north) -- (s4.west);        

\node (g1split) at ($(d1.south west) - (14mm, 0)$) [anchor=center, inner sep=0.37mm, outer sep=0mm, circle, fill=SkyBlue1] {};
\draw [arrows={- Stealth[]}, rounded corners=2pt, SkyBlue1, thick] (g1split.center) |- ($(d0.south east) - (0mm, 1.50mm)$);
\draw [arrows={- Stealth[]}, rounded corners=2pt, SkyBlue1, thick] (g1split.center) |- ($(d4.south east) - (0mm, 0.75mm)$);
\draw [arrows={- Stealth[]}, rounded corners=0pt, SkyBlue1, thick] (g1split.center) |- ($(d2.south east) - (0mm, 0.75mm)$)
node [pos=0.5, anchor=center, inner sep=0.37mm, outer sep=0mm, circle, fill=SkyBlue1] {};
\draw [arrows={ - Stealth[]}, SkyBlue1, thick] (g1.south) -- (d1.south west) 
node [pos=0.13, above=0.35mm, black] {$\hat{\underline{x}}_1$} 
node [pos=0.83, above=0.35mm, black] {real};

\node (g2split) at ($(d2.south west) - (19mm, 0)$) [anchor=center, inner sep=0.37mm, outer sep=0mm, circle, fill=SkyBlue2] {};
\draw [arrows={- Stealth[]}, rounded corners=2pt, SkyBlue2, thick] (g2split.center) |- ($(d0.south east) - (0mm, 0.0mm)$);
\draw [arrows={- Stealth[]}, rounded corners=2pt, SkyBlue2, thick] (g2split.center) |- ($(d4.south east) + (0mm, 0.75mm)$)
node [pos=0.83, above=0.35mm, black] {fake};
\draw [arrows={- Stealth[]}, rounded corners=0pt, SkyBlue2, thick] (g2split.center) |- ($(d1.south east) - (0mm, 0.75mm)$)
node [pos=0.5, anchor=center, inner sep=0.37mm, outer sep=0mm, circle, fill=SkyBlue2] {};
\draw [arrows={ - Stealth[]}, SkyBlue2, thick] (g2.south) -- (d2.south west) 
node [pos=0.13, above=0.35mm, black] {$\hat{\underline{x}}_2$} 
node [pos=0.83, above=0.35mm, black] {real};

\node (g4split) at ($(d4.south west) - (24mm, 0)$) [anchor=center, inner sep=0.37mm, outer sep=0mm, circle, fill=SkyBlue3] {};
\draw [arrows={- Stealth[]}, rounded corners=2pt, SkyBlue3, thick] (g4split.center) |- ($(d0.south east) + (0mm, 1.50mm)$)
node [pos=0.863, above=0.35mm, black] {fake};
\draw [arrows={- Stealth[]}, rounded corners=0pt, SkyBlue3, thick] (g4split.center) |- ($(d1.south east) + (0mm, 0.75mm)$)
node [pos=0.5, anchor=center, inner sep=0.37mm, outer sep=0mm, circle, fill=SkyBlue3] {}
node [pos=0.863, above=0.35mm, black] {fake};
\draw [arrows={- Stealth[]}, rounded corners=0pt, SkyBlue3, thick] (g4split.center) |- ($(d2.south east) + (0mm, 0.75mm)$)
node [pos=0.5, anchor=center, inner sep=0.37mm, outer sep=0mm, circle, fill=SkyBlue3] {}
node [pos=0.865, above=0.35mm, black] {fake};
\draw [arrows={ - Stealth[]}, SkyBlue3, thick] (g4.south) -- (d4.south west) 
node [pos=0.13, above=0.35mm, black] {$\hat{\underline{x}}_K$} 
node [pos=0.83, above=0.35mm, black] {real};

\draw [decorate, decoration={brace, aspect=0.5, raise=20mm}] (d1.bottom left corner) -- (d4.bottom right corner)
node[pos=0.5, right, rotate=-90, anchor=south, yshift=22mm] {Supplementary discriminators};
\draw [decorate, decoration={brace, aspect=0.5, raise=17mm}] (g4.bottom left corner) -- (g1.bottom right corner)
node[pos=0.5, right, rotate=-90, anchor=north, yshift=-19mm] {Generators and latent variables};
\node at (s0.east) [rotate=-90, anchor=south, yshift=1.5mm, align=center] {Adversarial \\ discriminator};
\node at (g0.west) [rotate=-90, anchor=north, yshift=-4.0mm, align=center] {Real data \\ distribution};

\end{tikzpicture}
\caption{{\small A diagram of the proposed multi-generator GAN architecture. Multiple inputs to each discriminator is essentially aggregation of sample from different distributions into a single batch.}}
\label{fig:model-architecture}


==> Selective Sampling and Mixture Models in Generative Adversarial Networks/literature.tex <==
List of references:
   
   
... PRINTED
1. Generative Image Modeling using Style and Structure Adversarial Networks ... Wang 2016
2. Generative Adversarial Nets ... Goofellow 2014
3. Deep Generative Image Models using a Laplacian Pyramid of Adversarial Networks ... Denton 2015
4. On distinguishability criteria for estimating generative models ... Goodfellow 2015
1. Energy-Based GAN (EBGAN) ... Zhao 2017
1. Deep Directed Generative Models with Energy-Based Probability Estimation ... Kim 2016
1. Unsupervised Representation Learning with Deep Convolutional Generative Adversarial Networks ... Radford 2015
1. Pixel-level domain transfer ... Yoo 2016
1. Unsupervised and Semi-Supervised Learning with Categorical Generative Adversarial Networks ... Springenberg 2015
1. Conditional Generative Adversarial Nets for Convolutional Face Generation ... Gauthier 2015
1. Conditional Generative Adversarial Nets ... Mirza 2014
1. Deep Multi-Scale Video Prediction Beyond Mean Square Error ... Mathieu 2015
1. Generating Images with Recurrent Adversarial Networks ... Im 2016
1. Adversarial Auto Encoders ... Machzani 2015
1. Auto-encoding beyond pixels using a learned Similarity Metric ... Larsen 2015
1. Generating Images with Perceptual Similarity Metrics based on Deep Networks ... Dosovitskiy 2016
1. Improved Techniques for Training GANs ... Salimans 2016
1. Generative Visual Manipulation on the Natural Image Manifold ... Zhu 2016
1. Context Encoder: Feature Learning by Inpainting ... Pathak 2016
1. Generating Video with Scene Dynamics ... Vondrick 2016
1. Learning a Probabilistic Latent Space of Object Shapes vis 3D Generative Adversarial Modeling ... Wu 2016

... UNSURE


==> Selective Sampling and Mixture Models in Generative Adversarial Networks/packages_01.tex <==
% \usepackage[export]{adjustbox}
% The package provides several macros to adjust boxed content. One purpose is to supplement the standard graphics package, which defines the macros \resizebox, \scalebox and \rotatebox , with the macros\trimbox and \clipbox. The main feature is the general \adjustbox macro which extends the ?key=value? interface of \includegraphics from the graphics package and applies it to general text content. Additional provided box macros are \lapbox, \marginbox, \minsizebox, \maxsizebox and \phantombox. All macros use the collectbox package to read the content as a box and not as a macro argument. This allows for all forms of content including special material like verbatim content. A special feature of collectbox is used to provide matching environments with the identical names as the macros.

% \usepackage[ruled,vlined]{algorithm2e}
%\usepackage[lined,plain,linesnumbered,commentsnumbered,figure,noline]{algorithm2e}
% Algorithm2e is an environment for writing algorithms. An algorithm becomes a floating object (like fig­ure, table, etc.). The package provides macros that allow you to create different keywords, and a set of predefined key words is provided; you can change the typography of the keywords. The package allows vertical lines delimiting a block of instructions in an algorithm, and defines different sorts of algorithms such as Procedure or Function; the name of these functions may be reused in the text or in other algo­rithms.

%\usepackage{algorithmic}
% algorithmic.sty was written by Peter Williams and Rogerio Brito. This package provides an algorithmic environment fo describing algorithms. You can use the algorithmic environment in-text or within a figure environment to provide for a floating algorithm. Do NOT use the algorithm floating environment provided by algorithm.sty (by the same authors) or algorithm2e.sty (by Christophe Fiorio) as IEEE does not use dedicated algorithm float types and packages that provide these will not provide correct IEEE style captions. The latest version and documentation of algorithmic.sty can be obtained at: http://www.ctan.org/tex-archive/macros/latex/contrib/algorithms/  There is also a support site at: http://algorithms.berlios.de/index.html  Also of interest may be the (relatively newer and more customizable) algorithmicx.sty package by Szasz Janos: http://www.ctan.org/tex-archive/macros/latex/contrib/algorithmicx/

%\usepackage{algorithmicx}
% Algorithmicx provides a flexible, yet easy to use, way for inserting good looking pseudocode or source code in your papers. It has built in support for Pseudocode, Pascal and C, and offers powerful means to create definitions for any programming language. The user can adapt a Pseudocode style to his native language. This package provides many possibilities to customize the layout of algorithms. You can use one of the predefined layouts (pseudocode, pascal, C, and others), with or without modifications, or you can define a completely new layout for your specific needs.

\usepackage{amsfonts}
% An extended set of fonts for use in mathematics, including: extra mathematical symbols; blackboard bold letters (uppercase only); fraktur letters; subscript sizes of bold math italic and bold Greek letters; subscript sizes of large symbols such as sum and product; added sizes of the Computer Modern small caps font; cyrillic fonts (from the University of Washington); Euler mathematical fonts. All fonts are proA­vided as Adobe Type 1 files, and all except the Euler fonts are provided as METAFONT source. The distribution also includes the canonical Type 1 versions of the Computer Modern family of fonts.  Plain TeX and LaTeX macros for using the fonts are provided.

\usepackage{amsmath}
% \usepackage[cmex10]{amsmath}	
% The package provides the principal packages in the AMS-LaTeX distribution. It adapts for use in LaTeX most of the mathematical features found in AMS-TeX; it is highly recommendsd as an adjunct to serious mathematical typesetting in LaTeX. When amsmath is loaded, AMS-LaTeX packages amsbsy (for bold symbols), amsopn (for operator names) and amstext (for text embdedded in mathematics) are also loaded. Amsmath is part of the LaTeX required distribution; however, several contributed packages add still furA­ther to its appeal; examples are empheq, which provides functions for decorating and highlighting mathA­ematics, and ntheorem, for specifying theorem (and similar) definitions. % A popular package from the American Mathematical Society that provides many useful and powerful commands for dealing with mathematics. If using it, be sure to load this package with the cmex10 option to ensure that only type 1 fonts will utilized at all point sizes. Without this option, it is possible that some math symbols, particularly those within footnotes, will be rendered in bitmap form which will result in a document that can not be IEEE Xplore compliant! Also, note that the amsmath package sets \interdisplaylinepenalty to 10000 thus preventing page breaks from occurring within multiline equations. Use: \interdisplaylinepenalty=2500 after loading amsmath to restore such page breaks as IEEEtran.cls normally does. amsmath.sty is already installed on most LaTeX systems. The latest version and documentation can be obtained at: http://www.ctan.org/tex-archive/macros/latex/required/amslatex/math/

% \usepackage{amssymb}
% A big list of symbols

%\usepackage{appendix}
% The appendix package provides various ways of formatting the titles of appendices. Also (sub)appenA­dices environments are provided that can be used, for example, for per chapter/section appendices. The word â??Appendixâ?? or similar can be prepended to the appendix number for article class documents. The word â??Appendicesâ?? or similar can be added to the table of contents before the appendices are listed. The word â??Appendicesâ?? or similar can be typeset as a \part-like heading (page) in the body. An appendices environment is provided which can be used instead of the \appendix command.

% \usepackage{array}
% An extended implementation of the array and tabular environments which extends the options for column formats, and provides "programmable" format specifications. This package is part of the tools bundle in the LaTeX required distribution. Frank Mittelbach's and David Carlisle's array.sty patches and improves the standard LaTeX2e array and tabular environments to provide better appearance and additional user controls. As the default LaTeX2e table generation code is lacking to the point of almost being broken with respect to the quality of the end results, all users are strongly advised to use an enhanced (at the very least that provided by array.sty) set of table tools. array.sty is already installed on most systems. The latest version and documentation can be obtained at: http://www.ctan.org/tex-archive/macros/latex/required/tools/

%\ifthenelse{\equal{\doclang}{german}}{\usepackage[ngerman]{babel}}{}
% The package manages culturally-determined typographical (and other) rules, and hyphenation patterns for a wide range of languages. A document may select a single language to be supported, or it may seA­lect several, in which case the document may switch from one language to another in a variety of ways. Babel uses contributed configuration files that provide the detail of what has to be done for each lanA­guage. Users of Xâ??TeX are advised to use polyglossia rather than Babel.

%\usepackage{bigstrut}
%\bigstrut produces a strut which is \bigstrutjot higher, lower, or both, than the standard array/table strut. Use it in table entries that are adjacent to an \hline, to leave an extra bit of space. Note that the tabls package does the job automatically, and the booktabs package has a completely dif­ferent mechanism for dealing with the problem, which obviates the need for manual adjustment.

% \usepackage{booktabs}
% The package enhances the quality of tables in LATEX, providing extra commands as well as behind-the-scenes optimisation. Guidelines are given as to what constitutes a good table in this context. From version 1.61, the package offers longtable compatibility.

\usepackage{bm}
% The bm package defines a command \bm which makes its argument bold. The argument may be any maths object from a single symbol to an expression. This is closely related to the specification of the \boldsymbol command in AMS-LaTeX, but \bm is rather more careful in the way it does things. The package is part of the tools bundle in the LaTeX required distribution.

%\usepackage{booktabs}
% The package enhances the quality of tables in LaTeX, providing extra commands as well as behind-the-scenes optimisation. Guidelines are given as to what constitutes a good table in this context. From ver­sion 1.61, the package offers longtable compatibility.

\usepackage{caption}
% \usepackage[font={footnotesize}]{caption}	%\usepackage[format=hang]{caption} 	%\usepackage[caption=false]{caption}
% The caption package provides many ways to customise the captions in floating environments like figure and table, and cooperates with many other packages. Facilities include rotating captions, sideways capA­tions, continued captions (for tables or figures that come in several parts). A list of compatibility notes, for other packages, is provided in the documentation. The package also provides the â??caption outside floatâ?? facility, in the same way that simpler packages like capt-of do.  The package supersedes caption2.

%\usepackage[europeanresistors,americaninductors]{circuizz}
% The package provides a set of macros for naturally typesetting electrical and (somewhat less naturally, perhaps) electronic networks. It is designed as a tool that is easy to use, with a lean syntax, native to LaTeX, and directly supporting PDF output format. So is based on the very impressive pgf/TikZ package.
 
% \usepackage[final]{changes}
%\usepackage[draft, markup = underlined]{changes}
% The package allows the user to manually markup changes of text, such as additions, deletions, or replacements. Changed text is shown in a different colour; deleted text is crossed out. The package allows definition of additional authors and their associated colour. It also allows you to define a markup for authors or annotations. A bash script is provided for removing the changes.
 
%\usepackage[noadjust]{cite}
% cite.sty was written by Donald Arseneau V1.6 and later of IEEEtran pre-defines the format of the cite.sty package. \cite{} output to follow that of IEEE. Loading the cite package will result in citation numbers being automatically sorted and properly "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's \cite will automatically add leading space, if needed. Use cite.sty's noadjust option (cite.sty V3.8 and later) if you want to turn this off. cite.sty is already installed on most LaTeX systems. Be sure and use  version 4.0 (2003-05-27) and later if using hyperref.sty. cite.sty does not currently provide for hyperlinked citations. The latest version can be obtained at: http://www.ctan.org/tex-archive/macros/latex/contrib/cite/ The documentation is contained in the cite.sty file itself.

%\usepackage{cleveref}
% The package enhances LATEX's cross-referencing features, allowing the format of references to be determined automatically according to the type of reference. The formats used may be customised in the preamble of a document; babel support is available (though the choice of languages remains limited: currently Danish, Dutch, English, French, German, Italian, Norwegian, Russian, Spanish and Ukranian). The package also offers a means of referencing a list of references, each formatted according to its type. In such lists, it can collapse sequences of numerically-consecutive labels to a reference range.

%\usepackage{color}
% The color package provides both foreground (text, rules, etc.) and background colour management; it uses the device driver configuration mechanisms of the graphics package to determine how to control its ouptut. The package is part of the LaTeX graphics bundle.

%\usepackage{colortbl}
% This package implements a  flexibable mechanism for giving colured `panels' behind specied columns in a table. This package requires the array and color packages.

% \usepackage{dcolumn}

%\usepackage{doublespace}
% Double space environment. A LaTeX 2.09 package that defines a spacing environment which you can use anywhere in your docu­ment. This package should no longer be used: it has serious bugs, and is no longer maintained. It is super­seded by setspace.

% \usepackage{dsfont}
% A font based on Computer Modern Roman useful for typesetting the mathematical symbols for the natural numbers (N), whole numbers (Z), rational numbers (Q), real numbers (R) and complex numbers (C); coverage includes all Roman capital letters, ‘1’, ‘h’ and ‘k’. The font is available both as METAFONT source and in Adobe Type 1 format, and LATEX macros for its use are provided. The fonts appear in the blackboard bold sampler.

%	\let\labelindent\IEEElabelindent
%As IEEEtran.cls provides its own means to format lists, it might be better to read its documentation and template and use these methods instead of the enumitem module. Or, if using IEEEtran is not necessary, to switch to another documentclass. As IEEEtran.cls actually defines the \labelindent only for backwards compatibility reasons:: provide for legacy IED commands/lengths when possible the macro can be re-used without side-effects.
% Exporting to LaTeX, inserting the line::
%	\let\labelindent\relax
%before the call to enumitem (\usepackage{enumitem}) and running latex "by hand" works around the name clash.

% \let\labelindent\relax
% \usepackage{enumitem}
%This pack?age pro?vides user con?trol over the lay?out of the three ba?sic list en?vi?ron?ments: enu?mer?ate, item?ize and de?scrip?tion. It su?per?sedes both enu?mer?ate and md?wlist (pro?vid?ing well-struc?tured re?place?ments for all their fun?tion?al?ity), and in ad?di?tion pro?vides func?tions to com?pute the lay?out of la?bels, and to ?clone? the stan?dard en?vi?ron?ments, to cre?ate new en?vi?ron?ments with coun?ters of their own.

%\usepackage{epsfig}
% This package was developed as a general solution to the problem of including graphics in LaTeX 2.09; as such there are obsolete copies to be found on the web (though no longer on the archive). These old versions should not be used with current LaTeX. The current ‘preferred’ solution is the LaTeX graphicx package, but the graphics bundle does contain a version of epsfig for use with current LaTeX.

%\usepackage{eqparbox}
% Also of notable interest is Scott Pakin's eqparbox package for creating (automatically sized) equal width boxes - aka "natural width parboxes". Available at: http://www.ctan.org/tex-archive/macros/latex/contrib/eqparbox/

% \usepackage{etoolbox}
% The package is a toolbox of programming facilities geared primarily towards LATEX class and package authors. It provides LATEX frontends to some of the new primitives provided by e-TEX as well as some generic tools which are not strictly related to e-TEX but match the profile of this package. Note that the initial versions of this package were released under the name elatex. The package provides functions that seem to offer alternative ways of implementing some LATEX kernel commands; nevertheless, the package will not modify any part of the LATEX kernel.

% \usepackage{eucal}
% A package of the AMS which rovides more scripted font. The command \mathscr{#1}, it gives access to script capitals. For example, $\mathscr{MATHEMATIC}$%. If the eucal paage is used, the option [mathscr] provides both the standard \mathcal and the \mathscr commands, producing a different script font.

%\usepackage{fancyhdr}
% The package provides extensive facilities, both for constructing headers and footers, and for controlling their use (for example, at times when LATEX would automatically change the heading style in use).

% \usepackage[bottom]{footmisc}
% A collection of ways to change the typesetting of footnotes. The package provides means of changing the layout of the footnotes themselves (including setting them in ‘paragraphs’ — the para option), a way to number footnotes per page (the perpage option), to make footnotes disappear in a ‘moving’ argument (stable option) and to deal with multiple references to footnotes from the same place (multiple option). The package also has a range of techniques for labelling footnotes with symbols rather than numbers. Some of the functions of the package are overlap with the functionality of other packages. The para option is also provided by the manyfoot and bigfoot packages, though those are both also portmanteau packages. (Don't be seduced by fnpara, whose implementation is improved by the present package.) The perpage option is also offered by footnpag and by the rather more general-purpose perpage}

\usepackage{float}
% Improves the interface for defining floating objects such as figures and tables. Introduces the boxed float, the ruled float and the plaintop float. You can define your own floats and improve the behaviour of the old ones. The package also provides the H float modifier option of the obsolete here package. You can select this as automatic default with \floatplacement{figure}{H}.

%\usepackage[T1]{fontenc}
% The package allows the user to select font encodings, and for each encoding provides an interface to â??font-encoding-specificâ?? commands for each font. Its most powerful effect is to enable hyphenation to opA­erate on texts containing any character in the font. The package supersedes t1enc; it is distributed as part of the latex distribution.

%\usepackage{fixltx2e}
% fixltx2e, the successor to the earlier fix2col.sty, was written by Frank Mittelbach and David Carlisle. This package corrects a few problems in the LaTeX2e kernel, the most notable of which is that in current LaTeX2e releases, the ordering of single and double column floats is not guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow asingle column figure to be placed prior to an earlier double column figure. The latest version and documentation can be found at: http://www.ctan.org/tex-archive/macros/latex/base/

%\usepackage{fullpage}

%\usepackage[a3paper, left = 57.5mm, right = 57.5mm, top = 40mm, bottom = 135mm]{geometry}
%\usepackage[left = 15mm, top = 19mm, right = 15mm, bottom = 40mm]{geometry}	
%\usepackage[margin = 1.5cm, includefoot, footskip = 30pt]{geometry}	
%\usepackage[right = 19.91mm, left = 19mm, top = 19mm, bottom = 31mm]{geometry}
%\usepackage[right = 0.51in, left = 0.51in, top = 0.75in, bottom = 1.69in]{geometry}
%\usepackage[vcentering,dvips]{geometry}
% The package provides an easy and flexible user interface to customize page layout, implement­ing auto-centering and auto-balancing mechanisms so that the users have only to give the least description for the page layout. For example, if you want to set each margin 2cm without header space, what you need is just \usepackage[margin=2cm,nohead]{geometry}. The package knows about all the standard paper sizes, so that the user need not know what the nominal ‘real’ dimensions of the paper are, just its standard name (such as a4, letter, etc.). An important feature is the package’s ability to communicate the paper size it's set up to the output (whether via DVI \specials or via direct interaction with PDF(La)TeX).

%\usepackage[acronym, toc, style=super4col, nonumberlist]{glossaries}
%\usepackage{glossaries}

%\usepackage{graphics}
% The package was designed to accommodate all needs for inclusion of graphics in LaTeX docu­ments, replacing many earlier packages used in LaTeX 2.09. The package aims to give a con­sistent interface to including the file types that are understood in your output, by use of ‘printer drivers’ (now known, simply, as ‘drivers’). The distribtion of the package contains sev­eral drivers, but others (for example, pdfTeX) are distributed separately. The package also of­fers several means of manipulating graphics in the course of inserting them into a document (for example, rotation and scaling). For extended documentation see epslatex. The package is part of the graphics bundle, which is one of the collections in the LaTeX ‘re­quired’ set of packages. % graphicx was written by David Carlisle and Sebastian Rahtz. It is required if you want graphics, photos, etc. graphicx.sty is already installed on most LaTeX systems. The latest version and documentation can be obtained at: http://www.ctan.org/tex-archive/macros/latex/required/graphics/  Another good source of documentation is "Using Imported Graphics in LaTeX2e" by Keith Reckdahl which can be found as epslatex.ps or epslatex.pdf at: http://www.ctan.org/tex-archive/info/  latex, and pdflatex in dvi mode, support graphics in encapsulated postscript (.eps) format. pdflatex in pdf mode supports graphics in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure that all non-photo figures use a vector format (.eps, .pdf, .mps) and not a bitmapped formats (.jpeg, .png). IEEE frowns on bitmapped formats which can result in "jaggedy"/blurry rendering of lines and letters as well as large increases in file sizes. You can find documentation about the pdfTeX application at: http://www.tug.org/applications/pdftex
%\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
%\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
%\fi

 
\usepackage{graphicx}
% The package builds upon the graphics package, providing a key-value interface for optional arguments to the \includegraphics command. This interface provides facilities that go far beyond what the graphics package offers on its own. For extended documentation, see epslatex. The package is part of the graphics bundle, which is one of the collections in the LaTeX â??requiredâ?? set of packages.

%\usepackage[bookmarks=false, draft]{hyperref}
% \usepackage{hyperref}
% The hyperref package is used to handle cross-referencing commands in LaTeX to produce hypertext links in the document. The package provides backends for the \special set defined for HyperTeX DVI processors; for embedded pdfmark commands for processing by Acrobat Distiller (dvips and Y&Yâ??s dvipsone); for Y&Yâ??s dviwindo; for PDF control within pdfTeX and dvipdfm; for TeX4ht; and for VTeXâ??s pdf and HTML backends. The package is distributed with the backref and nameref packages, which make use of the facilities of hyperref. The package depends on the authorâ??s kvoptions, ltxcmdsand refcount packages.

%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional compilation based on whether the output is pdf or dvi.          Usage:	\ifpdf	% pdf code	\else	% dvi code	\fi . The latest version of ifpdf.sty can be obtained from:	http://www.ctan.org/tex-archive/macros/latex/contrib/oberdiek/ . Also, note that IEEEtran.cls V1.7 and later provides a builtin \ifCLASSINFOpdf conditional that works the same way. When switching from latex to pdflatex and vice-versa, the compiler may have to be run twice to clear warning/error messages.

% \usepackage{ifthen}
% The package's basic command is \ifthenelse, which can use a wide array of tests. Also provided is a simple loop command \whiledo. Ifthen is a separate package within the LaTeX distribution; while it will always be present in a LaTeX distriA­bution, a \usepackage command is always needed to load it.

% \usepackage{indentfirst}
% This minimalist package is part of the tools bundle in the LaTeX required distribution.

%\usepackage[latin1]{inputenc}
% The package translates various standard and other input encodings into a â??LaTeX internal languageâ??. The internal language is expressed entirely in TeX's base encoding (standard ASCII printable characters, carriage control tokens and TeX control sequences, the latter mostly defined by LaTeX). The package is part of the LaTeX distribution.

%\usepackage{lastpage}
% Reference the number of pages in your LATEX document through the introduction of a new label which can be referenced like \pageref{LastPage} to give a reference to the last page of a document. It is particularly useful in the page footer that says: Page N of M.

%\usepackage{latexdiff}
% Latexdiff is a Perl script for visual mark up and revision of significant differences between two LATEX files. Various options are available for visual markup using standard LATEX packages such as color. Changes not directly affecting visible text, for example in formatting commands, are still marked in the LATEX source. A rudimentary revision facilility is provided by another Perl script, latexrevise, which accepts or rejects all changes. Manual editing of the difference file can be used to override this default behaviour and accept or reject selected changes only.

% \usepackage{lipsum}

%\usepackage{longtable}
% Allow tables to flow over page boundaries. Longtable allows you to write tables that continue to the next page. You can write captions within the ta?ble (typically at the start of the table), and headers and trailers for pages of table. Longtable arranges that the columns on successive pages have the same widths. This last contrasts with the superficially similar supertabular package. Longtable (unlike supertabular) modifies the output routine, and consequently won't work in a multicol?umn environment (or in other circumstances where the output routine has been critically altered); it also fails in twocolumn pages. This package is part of the tools bundle in the LaTeX required distribution.

%\usepackage{lscape}
% Modifies the margins and rotates the page contents but not the page number. Useful, for exam­ple, with large multipage tables, as it is compatible with longtable and supertabular. Note that the package makes no special provision for PDF output, where in principle a single page can be shown at full landscape width; such an effect may be achieved using the pdflscape package instead. The package is part of the graphics bundle, which is one of the collections in the LaTeX ‘re­quired’ set of packages.
 
%\usepackage{mathdots}
% This package provides vertical dots and diagonal dots in math, slanting in either direction. It should work equally well in LATEX or plain TEX. It improves on the default definitions of plain TEX and LATEX. Similar improvements are provided for the triple and quadruple dot accents of AMSTEX/AMSLATEX. 
 
% \usepackage{mathtools}
%Math­tools pro­vides a se­ries of pack­ages de­signed to en­hance the ap­pear­ance of doc­u­ments con­tain­ing a lot of math­e­mat­ics. The main back­bone is ams­math, so those un­fa­mil­iar with this re­quired part of the LATEX sys­tem will prob­a­bly not find the pack­ages very use­ful. Math­tools pro­vides many use­ful tools for math­e­mat­i­cal type­set­ting. It is based on ams­math and fixes var­i­ous de­fi­cien­cies of ams­math and stan­dard LATEX. It pro­vides: Ex­ten­si­ble sym­bols, such as brack­ets, ar­rows, har­poons, etc.; Var­i­ous sym­bols such as \coloneqq (:=); Easy cre­ation of new tag forms; Show­ing equa­tion num­bers only for ref­er­enced equa­tions; Ex­ten­si­ble ar­rows, har­poons and hookar­rows; Starred ver­sions of the ams­math ma­trix en­vi­ron­ments for spec­i­fy­ing the col­umn align­ment; More build­ing blocks: mult­lined, cases-like en­vi­ron­ments, new gath­ered en­vi­ron­ments; Maths ver­sions of \make­box, \llap, \rlap etc.; Cramped math styles; and more...

%\usepackage{mdwmath}

%\usepackage{mdwtab}
% Also highly recommended is Mark Wooding's extremely powerful MDW tools, especially mdwmath.sty and mdwtab.sty which are used to format equations and tables, respectively. The MDWtools set is already installed on most LaTeX systems. The lastest version and documentation is available at: http://www.ctan.org/tex-archive/macros/latex/contrib/mdwtools/

% \usepackage{moresize}
% A package for using font sizes up to 35.88pt, for example with the EC fonts. New commands \HUGE and \ssmall for selecting font sizes are provided together with some options working around current LATEX2ε shortcomings in using big font sizes. The package also provides options for improving the typesetting of paragraphs (or headlines) with embedded math expressions at font sizes above 17.28pt.

% \usepackage{multicol}
% Intermix single and multiple columns. Multicol defines a multicols environment which typesets text in multiple columns (up to a maximum of 10), and (by default) balances the end of each column at the end of the environment. The package en?ables you to switch between any (permitted) number of columns at will: there is no imposed "clear page" operation, as there is in unadorned LaTeX at a switch between \onecolumn and \twocolumn sections. The multicolumn environment can also be used inside a box, thus allowing multicolumned insets in text. Multicol patches the output routine, and may clash with other packages that do the same (e.g., longtable); furthermore, there is no provision for single column floats inside a multicolumn environment, so figures and tables must be coded in-line (using, for example, the H modifier of the float package). The package is part of the tools bundle in the LaTeX required distribution.
 
% \usepackage{multirow}
% The package has a lot of flexibility, including an option for specifying an entry at the “natural” width of its text. The package is distributed with the bigdelim and bigstrut packages, which can be used to ad­vantage with \multirow cells.

% \usepackage[square,numbers,sort&compress]{natbib}
% The bundle provides a package that implements both author-year and numbered references, as well as much detailed of support for other bibliography use. Also Provided are versions of the standard BibTeX styles that are compatible with natbibâ??plainnat, unsrtnat, abbrnat. The bibliography styles produced by custom-bib are designed from the start to be compatible with natbib.

%\usepackage{parskip}
% Simply changing \parskip and \parindent leaves a layout that is untidy; this package (though it is no substitute for a properly-designed class) helps alleviate this untidiness

%\usepackage{pdfcomment}
% For a long time pdfLaTeX has offered the command \pdfannot for inserting arbitrary PDF annotations. However, the command is presented in a form where additional knowledge of the definition of the PDF format is indispensable. This package is an answer to the ? occasional ? questions in newsgroups, about how one could use the comment function of Adobe Reader. At least for the writer of LaTeX code, the package offers a convenient and user-friendly means of using \pdfannot to provide comments in PDF files. Since version v1.1, pdfcomment.sty also supports LaTeX ? dvips ? ps2pdf, LaTeX ? dvipdfmx, and XeLaTeX. Unfortunately, support of PDF annotations by PDF viewers is sparse to nonexistent. The reference viewer for the development of this package is Adobe Reader. The author is Josef Kleber. The package is Copyright ? 2008-2012 Josef Kleber.

% \usepackage{pdfpages}
% This package simplifies the inclusion of external multi-page PDF documents in LATEX documents. Pages may be freely selected and similar to psnup it is possible to put several logical pages onto each sheet of paper. Furthermore a lot of hypertext features like hyperlinks and article threads are provided. The package supports pdfTEX (pdflatex) and VTEX. With VTEX it is even possible to use this package to insert PostScript files, in addition to PDF files.

% \usepackage{perpage}
% The package provides a mechanism to reset counters per page and/or keep their occurences sorted in order of appearance on the page. The package also defines a command \MakePerPage that designates a counter to be reset per page. For example \MakePerPage[2]{footnote} will cause footnote numbers to start at 2 at the start of every page (the optional argument defaults to 1). The machanism may require multiple passes to work; LATEX gives the usual changed label warning if this is necessary. The package is distributed as part of the bigfoot bundle.

%\usepackage{pgf-pie}
% pgf-pie is a LaTeX package for drawing pie chart (and variant charts). As stated by its name, it is based on a very popular graphic package PGF/TikZ. This document presents the usage of pgf-pie and collects some pie charts as examples. pgf-pie can be downloaded from http://code.google.com/p/pgf-pie/.

% \usepackage{pgfplots}
% PGFPlots draws high-quality function plots in normal or logarithmic scaling with a user-friendly interface directly in TeX. The user supplies axis labels, legend entries and the plot coordinates for one or more plots and PGFPlots applies axis scaling, computes any logarithms and axis ticks and draws the plots, supporting line plots, scatter plots, piecewise constant plots, bar plots, area plots, mesh-- and surface plots and some more. Pgfplots is based on PGF/TikZ (pgf); it runs equally for LaTeX/TeX/ConTeXt.

%\usepackage{pgfplotstable}
% Pgfplotstable displays numerical tables rounded to desired precision in various display formats (for example scientific format, fixed point format or integer), using TeX’s mathematical facili­ties for pretty printing. Furthermore, it provides methods for table postprocessing.

%\usepackage{placeins}
% Defines a \FloatBarrier command, beyond which floats may not pass; useful, for example, to ensure all floats for a section appear before the next \section command.

%\usepackage{rotating}
% Rotation tools, including rotated full-page floats. A package built on the standard LaTeX graphics package to perform all the different sorts of rotation one might like, including complete figures and tables with their captions. If you want continuous text (i.e., more than one page) set in landscape mode, use the lscape package in­stead. The rotating packages only deals in rotated boxes (or floats, which are themselves boxes), and boxes always stay on one page. If you need to use the facilities of the float in the same document, load rotating.sty via rotfloat, which smooths the path between the rotating and float packages.

%\usepackage{rotfloat}
% Rotate floats. The float package provides commands to define new floats of various styles (plain, boxed, ruled, and userdefined ones); the rotating package provides new environments (sidewaysfigure and side?waystable) which are rotated by 90 or 270 degrees. But what about new rotated floats, e.g. a rotated ruled one? This package makes this possible; it builds a bridge between the two packages and ex?tends the commands from the float package to define rotated versions of the new floats, too.

%\usepackage[headsepline]{scrpage2}
% koma-script – A bundle of versatile classes and packages. The KOMA-Script bundle provides drop-in replacements for the article/report/book classes with empha­sis on typography and versatility. There is also a letter class, different from all other letter classes. The bundle also offers: – a package for calculating type areas in the way laid down by the typographer Jan Tschichold, – a package for easily changing and defining page styles, – a package scrdate for get­ting not only the current date but also the name of the day, and – a package scrtime for getting the cur­rent time. All these packages may be used not only with KOMA-Script classes but also with the standard classes. Since every package has its own version number, the version number quoted only refers to the version of scrbook, scrreprt, scrartcl, scrlttr2 and typearea. These are the main parts of the bundle.

% \usepackage[nodisplayskipstretch]{setspace}
% Set space between lines. Provides support for setting the spacing between lines in a document. Package options include sin­glespacing, onehalfspacing, and doublespacing. Alternatively the spacing can be changed as required with the \singlespacing, \onehalfspacing, and \doublespacing commands. Other size spacings also avail­able.

%\usepackage{showframe}
% The package shows a (simple, uncluttered) diagram of the page layout; similar (but more complex-looking) diagrams may be obtained from the layouts and geometry packages. The package is available as part of the eso-pic distribution.

% \usepackage{siunitx}

\usepackage{soul}
%Provides hyphenatable spacing out (letterspacing), underlining, striking out, etc., using the TEX hyphenation algorithm to find the proper hyphens automatically. The package also provides a mechanism that can be used to implement similar tasks, that have to treat text syllable by syllable. This is shown in two examples. The package itself does not support UTF-8 input in ordinary (PDF)LATEX; some UTF-8 support is offered by package soulutf8


\usepackage{spconf}
% A package for formatting the ICASSP 2015 paper ...

% \usepackage{stackengine}
% The package provides a versatile way to stack objects vertically in a variety of customizable ways. A number of useful macros are provided, all of which make use of the stackengine core.

% \usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e the ability to do double column floats at the bottom of the page as well as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in LaTeX2e). It also provides a command:\fnbelowfloat to enable the placement of footnotes below bottom floats (the standard LaTeX2e kernel puts them above bottom floats). This is an invasive package which rewrites many portions of the LaTeX2e float routines. It may not work with other packages that modify the LaTeX2e float routines. The latest version and documentation can be obtained at: http://www.ctan.org/tex-archive/macros/latex/contrib/sttools/ Documentation is contained in the stfloats.sty comments as well as in the presfull.pdf file. Do not use the stfloats baselinefloat ability as IEEE does not allow \baselineskip to stretch. Authors submitting work to the IEEE should note that IEEE rarely uses double column equations and that authors should try to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty packages (also by Sigitas Tolusis) as IEEE does not format its papers in such ways.

% \usepackage{subcaption}
% Support for sub-captions. The package provides a means of using facilities analagous to those of the caption package, when writ­ing captions for subfigures and the like. The package is distributed with caption.

%\usepackage{subfig}	%\usepackage[font=footnotesize]{subfig}
% Figures broken into subfigures. The package provides support for the manipulation and reference of small or ‘sub’ figures and tables within a single figure or table environment. It is convenient to use this package when your subfigures are to be separately captioned, referenced, or are to be included in the List-of-Figures. A new \subfigure command is introduced which can be used inside a figure environment for each subfigure. An optional first argument is used as the caption for that subfigure. This package supersedes the subfigure package (which is longer maintained). The name was changed since the package is completely backward compatible with the older package The major advantage to the new package is that the user interface is keyword/value driven and easier to use. To ease the transi­tion from the subfigure package, the distribution it includes a configuration file (subfig.cfg) which nearly emulates the subfigure package. The functionality of the package is provided by the (more recent still) subcaption package. subfig.sty, also written by Steven Douglas Cochran, is the modern replacement for subfigure.sty. However, subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty which will override IEEEtran.cls handling of captions and this will result in nonIEEE style figure/table captions. To prevent this problem, be sure and preload caption.sty with its "caption=false" package option. This is will preserve IEEEtran.cls handing of captions. Version 1.3 (2005/06/28) and later (recommended due to many improvements over 1.2) of subfig.sty supports the caption=false option directly: \usepackage[caption=false,font=footnotesize]{subfig}. The latest version and documentation can be obtained at: http://www.ctan.org/tex-archive/macros/latex/contrib/subfig/ The latest version and documentation of caption.sty can be obtained at: http://www.ctan.org/tex-archive/macros/latex/contrib/caption/


%\usepackage{subfigure}	%\usepackage[tight,footnotesize]{subfigure}
% Deprecated, Deprecated, Deprecated: Figures divided into subfigures. Provides support for the manipulation and reference of small or ‘sub’ figures and tables within a single figure or table environment. It is convenient to use this package when your subfigures are to be sepa­rately captioned, referenced, or are to be included in the List-of-Figures. A new \subfigure command is introduced which can be used inside a figure environment for each subfigure. An optional first argument is used as the caption for that subfigure. The package is now considered obsolete: it was superseded by subfig, but users may find the more re­cent subcaption package more satisfactory. subfigure.sty was written by Steven Douglas Cochran. This package makes it easy to put subfigures in your figures. e.g., "Figure 1a and 1b". For IEEE work, it is a good idea to load it with the tight package option to reduce the amount of white space around the subfigures. subfigure.sty is already installed on most LaTeX systems. The latest version and documentation can be obtained at: http://www.ctan.org/tex-archive/obsolete/macros/latex/contrib/subfigure/ subfigure.sty has been superceeded by subfig.sty.

% \usepackage{tabu}

% \usepackage{tabularx}

% \usepackage{textcomp}
% LaTeX support for the Text Companion fonts. The package supports the Text Companion fonts, which provide many text symbols (such as baht, bullet, copyright, musicalnote, onequarter, section, and yen), in the TS1 encoding. Note that the package has been adopted as part of the LaTeX distribution; the reference here is to the original package, which is now little used (if at all).


%\usepackage{tikzscale}
% Resize pictures while respecting text size. The package extends the \includegraphics command to support tikzpictures. It allows scaling of TikZ images and PGFPlots to a given width or height without changing the text size.


    % Handle a bug when using the "titlesec" package (add the 'subparagraph' command)
%     \makeatletter\newcommand\subparagraph{\@startsection{subparagraph}{5}{\parindent}{3.25ex \@plus 1ex \@minus .2ex}{-1em}{\normalfont\normalsize\bfseries}}\makeatother
%\usepackage{titlesec}
% \usepackage[compact]{titlesec}
%     \let\subparagraph\relax
% A package providing an interface to sectioning commands for selection from various title styles. E.g., marginal titles and to change the font of all headings with a single command, also providing simple one-step page styles. Also includes a package to change the page styles when there are floats in a page. You may assign headers/footers to individual floats, too.
    

%\usepackage{tkz-kiviat}
% Draw Kiviat graphs. The package allows the user to draw Kiviat Graphs directly, or with data from an external file. The drawing is done with the help of pgfplots.
 
% \usepackage[color = yellow]{todonotes}
% The package lets the user mark things to do later, in a simple and and visually appealing way.  The package takes several options to enable customization / finetuning of the visual appearance. The package makes use of the tikz and xkeyval packages. 
 
%\usepackage{txfonts}
% Txfonts supplies virtual text roman fonts using Adobe Times (or URW NimbusRomNo9L) with some modified and additional text symbols in the OT1, T1, and TS1 encodings; maths alphabets using Times/URW Nimbus; maths fonts providing all the symbols of the Computer Modern and AMS fonts, including all the Greek capital letters from CMR; and additional maths fonts of various other symbols. The set is complemented by a sans-serif set of text fonts, based on Helvetica/NimbusSanL, and a monospace set. All the fonts are in Type 1 format (AFM and PFB files), and are supported by TeX metrics (VF and TFM files) and macros for use with LaTeX.

% \usepackage{url}
% Verbatim with URL-sensitive line breaks. The command \url is a form of verbatim command that allows linebreaks at certain characters or combi­nations of characters, accepts reconfiguration, and can usually be used in the argument to another com­mand. (The \urldef command provides robust commands that serve in cases when \url doesn't work in an argument.) The command is intended for email addresses, hypertext links, directories/paths, etc., which normally have no spaces, so by default the package ignores spaces in its argument. However, a package option “allows spaces”, which is useful for operating systems where spaces are a common part of file names. url.sty was written by Donald Arseneau. It provides better support for handling and breaking URLs. url.sty is already installed on most LaTeX systems. The latest version can be obtained at: http://www.ctan.org/tex-archive/macros/latex/contrib/misc/ Read the url.sty source comments for usage information. Basically, \url{my_url_here}.

%\usepackage{wrapfig}
% Allows figures or tables to have text wrapped around them. Does not work in combination with list enviA­ronments, but can be used in a parbox or minipage, and in twocolumn format. Supports the float packA­age. Alternatively you can use floatflt

\usepackage[x11names]{xcolor}
%xcolor provides easy driver-independent access to several kinds of colors, tints, shades, tones, and mixes of arbitrary colors by means of color expressions like \color{red!50!green!20!blue}. It allows to select a document-wide target color model and offers tools for automatic color schemes, conversion between twelve color models, alternating table row colors, color blending and masking, color separation, and color wheel calculations.

==> Selective Sampling and Mixture Models in Generative Adversarial Networks/packages_02.tex <==

%\usepackage[style=numeric-comp,natbib=true]{biblatex}
%\AtEveryBibitem{%
%	\clearfield{issn} % Remove issn
%	\clearfield{doi} % Remove doi
%	\ifentrytype{online}{}{\clearfield{url}} % Remove url except for @online
%}


% \usepackage{epstopdf}
%Epstopdf is a Perl script that converts an EPS file to an ‘encapsulated’ PDF file (a single page file whose media box is the same as the original EPS’s bounding box). The resulting file suitable for inclusion by PDFTEX as an image. The script is adapted to run both on Windows and on Unixalike systems. The script makes use of Ghostscript for the actual conversion to PDF. It assumes Ghostscript version 6.51 or later, and (by default) suppresses its automatic rotation of pages where most of the text is not horizontal. LATEX users may make use of the epstopdf package, which will run the epstopdf script “on the fly”, thus giving the illusion that PDFLATEX is accepting EPS graphic files.


\usepackage{tikz}
% Must be after the {xcolor} package if you need special options in the xcolor package.
% Create PostScript and PDF graphics in TeX. PGF is a macro package for creating graphics. It is platform- and format-independent and works to­gether with the most important TeX backend drivers, including pdftex and dvips. It comes with a user-friendly syntax layer called TikZ.  Its usage is similar to pstricks and the standard picture environment. PGF works with plain (pdf-)TeX, (pdf-)LaTeX, and ConTeXt. Unlike pstricks, it can produce either PostScript or PDF output.


==> Selective Sampling and Mixture Models in Generative Adversarial Networks/predocument.tex <==
%===============================================================================================================
%===========================================  Definitions  =====================================================
\newcommand{\on}{\emph{on}}
\newcommand{\off}{\emph{off}}
\newcommand{\plus}{\texttt{+}}
\newcommand{\minus}{\texttt{-}}
%=======================================  Defining Math Operators  =============================================
\DeclareMathOperator{\sign}{sign}
\newcommand{\argmin}{\operatornamewithlimits{arg\ min}}
\newcommand{\argmax}{\operatornamewithlimits{arg\ max}}
\newcommand{\abs}[1]{\left\vert\left\vert{#1}\right\vert\right\vert}
\newcommand{\card}[1]{\left\vert{#1}\right\vert}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert} % L-Norm that adjusts its size according to argument 
\newcommand{\JSD}{\text{D}_\text{JS}}
\newcommand{\KLD}{\text{D}_\text{KL}}
%\DeclareMathOperator{\argmax}{arg\!max}


\DeclareRobustCommand{\cvdots}{%e}
	\vcenter{%
		\baselineskip=4pt %spacing
		\hbox{.}\hbox{.}\hbox{.}
}}


%%===============================================================================================================
%%==================================  Spaces before and after equations  ========================================
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}

%%===============================================================================================================
%%===========================================  Selecting the title  =============================================
%\ifthenelse{\equal{\doclang}{german}}
%{
%	\def \langtitle{\deTitle}
%	\def \suptitle{\enTitle}	
%}
%{
%	\def \langtitle{\enTitle}
%	\def \suptitle{\deTitle}
%}


%%===============================================================================================================
%%========================================  Settings for PDF Document  ==========================================
%\pdfstringdef \studentPDF {\student} 
%\pdfstringdef \worktitlePDF {\langtitle}
%\pdfstringdef \worksubjectPDF {\worksubject}
%\pdfstringdef \keywordsPDF {\keywords}
%\hypersetup{pdfauthor=\studentPDF, 
%            pdftitle=\worktitlePDF,
%            pdfsubject=\worksubjectPDF,
%            pdfkeywords=\keywordsPDF}


%%===============================================================================================================
%%=====================================  Adjusting TikZ and PGF Plots  ==========================================
\usetikzlibrary{arrows.meta,
			    calc,
				decorations,
				decorations.pathmorphing,
				decorations.pathreplacing,
				positioning,
			    shapes.geometric}
%\usetikzlibrary{arrows.meta,
%				automata,
%				backgrounds,
%                calc,

%                intersections,
%                ocgx,
%				patterns,
%				petri,
%				positioning,
%			   %shadows,
%				shapes,
%				spy,
%				topaths}
%\pgfplotsset{compat=1.13}
%%\usepgfplotslibrary{groupplots}
%%\pgfplotsset{plot coordinates/math parser=false}
%%\usepgfplotslibrary{external}
%%\tikzexternalize
%% %PGF activate externalization.  The external library oers a convenient method to export every single tikzpicture into a separate .pdf (or .eps). Later runs of LATEX will simply include these graphics, thereby reducing typesetting time considerably. The library can also be used to submit documents to authors who do not even have pgfplots or TikZ installed. See pgfplots manual Section 7.1. To enable the system calls, we type pdflatex -shell-escape test
%
%
%%===============================================================================================================
%%================ Tabular booktabs rules' variables ============================================================
%%---------------------------------------------------------------------------------------------------------------
%\heavyrulewidth=0.11em
%\lightrulewidth=0.05em
%
%
%%===============================================================================================================
%%================ Headers' styles (chapter, section, subsection headers) and margins ===========================
%%---------------------------------------------------------------------------------------------------------------
%%\renewcommand{\chaptername}{}	% Supress the word "Chapter"
%%\renewcommand{\thechapter}{}	% Supress Chapter Numbering in margin
%%--------------------------------------------------------------------------------------------------------------- Requires the package "etoolbox"
%%\makeatletter % You can adjust the value in \vspace*{0pt}.
%%\patchcmd{\@makechapterhead}{50\p@}{0pt}{}{} % Supress spacing above \chappter header  
%%\patchcmd{\@makeschapterhead}{50\p@}{0pt}{}{} % Supress spacing above \chappter* header
%%\makeatother
%%--------------------------------------------------------------------------------------------------------------- Requires the package "titlesec"
%%\titleformat{\chapter}[hang]{\normalfont\huge\bfseries}{\thechapter.}{1em}{} 
%%\titlespacing{\chapter}{0pt}{0pt}{20pt}
%%\titlespacing{\section}{0pt}{0pt}{0pt}
%%\titlespacing{\subsubsection}{0pt}{15pt}{0pt}
%%---------------------------------------------------------------------------------------------------------------
%%\renewcommand\thesection{\arabic{section}.}										% Supress chapter numbering
%%\renewcommand\thesubsection{\arabic{section}.\arabic{subsection}}					% Supress chapter numbering
%%\renewcommand\thesection{\arabic{chapter}.\arabic{section}}							% Numbering format of sections
%%\renewcommand\thesubsection{\arabic{chapter}.\arabic{section}.\arabic{subsection}}	% Numbering format of subsections
%
%
%
%%===============================================================================================================
%%=======================================  Reset footnate per page  =============================================
%\MakePerPage{footnote}
%
%
%%===============================================================================================================
%%==========================================  Paragraph margins  ================================================
%\setlength{\parskip}{1mm} % Space between different paragraphs
%
%
%
%%===============================================================================================================
%%==========  The name, autorefname, and title of the algorithm listings (algorithm2e package)  =================
%\SetAlgorithmName{Algorithm}{Algorithm}{List of algorithms}
%
%
%
%%===============================================================================================================
%%============================================  Autoref Names  ==================================================
%\renewcommand*{\sectionautorefname}{Section}
%
%%\def\chapterautorefname{Chapter}	\def\sectionautorefname{Section} \def\figureautorefname{Figure} 
%%\def\equationautorefname{Equation} 	\def\partautorefname{Part} \def\AMSautorefname{Equation}
%%\def\appendixautorefname{Appendix}	\def\Itemautorefname{Item} \def\tableautorefname{Table}	
%%\def\subsubsectionautorefname{Subsubsection}	\def\subsectionautorefname{Subsection} 
%%\def\paragraphautorefname{Paragraph}	\def\Hfootnoteautorefname{Footnote} 
%%\def\subfigureautorefname{Figure} 	\def\theoremautorefname{Theorem} 
%%\def\algorithmautorefname{Figure} 	\def\theoremautorefname{Theorem} 
%%  \def\equationautorefname{Equation}%
%%  \def\footnoteautorefname{footnote}%
%%  \def\itemautorefname{item}%
%%  \def\figureautorefname{Figure}%
%%  \def\tableautorefname{Table}%
%%  \def\partautorefname{Part}%
%%  \def\appendixautorefname{Appendix}%
%%  \def\chapterautorefname{chapter}%
%%  \def\sectionautorefname{section}%
%%  \def\subsectionautorefname{subsection}%
%%  \def\subsubsectionautorefname{subsubsection}%
%%  \def\paragraphautorefname{paragraph}%
%%  \def\subparagraphautorefname{subparagraph}%
%%  \def\FancyVerbLineautorefname{line}%
%%  \def\theoremautorefname{Theorem}%
%%  \def\pageautorefname{page}%
%
%
%
%
%
%
%
%%
%%
%%\pagenumbering{gobble}
%%\setlength{\columnsep}{6mm}
%%%\setcounter{page}{100}
%%\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%%		T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%%
%%
%
%
%
%
%
%
%
%%===============================================================================================================
%%=====================================  Correcting Hyphenation  ================================================
%%\hyphenation{op-tical net-works semi-conduc-tor}
%%===============================================================================================================
%%=============================================  ?????????  =====================================================
%%\pagestyle{scrheadings}
%%\automark{chapter}
%%\clearscrheadfoot
%%\lehead[]{\pagemark~~\headmark}
%%\rohead[]{\headmark~~\pagemark}
%%\renewcommand{\chaptermark}[1]{\markboth {\sl \hspace{8mm}#1}{}}
%%\renewcommand{\sectionmark}[1]{\markright{\sl \thesection~#1\hspace{8mm}}}
%%\addtolength{\textheight}{15mm}
%%\parindent0ex
%%\renewcommand*{\pnumfont}{\normalfont\slshape} % Seitenzahl geneigt
%%\renewcommand*{\sectfont}{\bfseries} % Kapitelueberschrift nicht Helvetica
%\hypersetup{pdfstartview=FitH, bookmarks=true, bookmarksnumbered=true, bookmarksopen=false, breaklinks=false,
%		    citecolor = blue}
%\ifthenelse{\equal{\colortype}{color}}
%	{
%		\hypersetup{colorlinks = true, linkcolor = blue}
%	}
%	{
%		\ifthenelse{\equal{\colortype}{boxed}}
%		{}
%		{
%			\hypersetup{hidelinks=true}
%		}
%	}
%%===============================================================================================================
%%===========================================  Defining Colors  =================================================
%%\definecolor{darkblue}{rgb}{0,0,0.4}
%%===============================================================================================================
%%=====================================  User-defined declarations  =============================================
%%\newcommand{\matlab}{\textsc{Matlab}\raisebox{1ex}{\tiny{\textregistered}} }
%%\newcommand{\Z}{\mathbb{Z}}
%%\newcommand{\N}{\mathbb{N}}
%%\newcommand{\R}{\mathbb{R}}
%%\newcommand{\E}{\operatorname{E}}
%%\newcommand{\e}[1]{\operatorname{e}^{\,#1}}
%%\newcommand{\op}[1]{\operatorname{#1}}
%%\newcommand{\smtext}[1]{{\scriptscriptstyle\text{#1}}}
%%\newcommand{\bugfix}{\color{white}{\texttt{\symbol{'004}}}} 		% Bug-Fix Umlaute in Verbatim
%%\setlength\bigstrutjot{3pt}
%%\geometry{total={155mm,235mm}}
%%\newcommand{\plus}{\texttt{+}}
%%\newcommand{\minus}{\texttt{-}}
%%\pgfdeclareplotmark{o*}
%%{%
%%	\draw (0, 0) circle [radius = 1.75 pt];
%%	\fill (0, 0) circle [radius = 0.75 pt];
%%}
%
%%===============================================================================================================
%%======================================  Floats fractions of a page  ===========================================
%%\renewcommand{\topfraction}{1}
%%\renewcommand{\bottomfraction}{1}
%%\renewcommand{\textfraction}{0}
%%\setcounter{totalnumber}{10}
%%\setcounter{secnumdepth}{5}
%%\setcounter{tocdepth}{5}
%%\setlength{\parindent}{0.5cm}
%%===============================================================================================================
%%========================================  List of Symbols Glossary  ===========================================
%% Define a new glossary type
%%\newglossary[slg]{symbols}{sym}{sbl}{List of Symbols}
%%Den Punkt am Ende jeder Beschreibung deaktivieren
%%\renewcommand*{\glspostdescription}{}
%%Glossar-Befehle anschalten
%%\makeglossaries
%%Diese Befehle sortieren die Einträge in den
%%einzelnen Listen:
%%TeXmaker
%%makeindex -s %.ist -t %.alg -o %.acr %.acn
%%makeindex -s %.ist -t %.slg -o %.sym %.sbl
%%makeindex -s %.ist -t %.glg -o %.gls %.glo
%%TeXnicCenter
%%makeindex -s %tm.ist -t %tm.alg -o %tm.acr %tm.acn
%%makeindex -s %tm.ist -t %tm.slg -o %tm.sym %tm.sbl
%%makeindex -s %tm.ist -t %tm.glg -o %tm.gls %tm.glo
%%\input{./bib/glossary.tex}
%
%%\setlength{\marginparwidth}{4.5cm}
%%\presetkeys{todonotes}{fancyline, linecolor = green!30, backgroundcolor=yellow!70, bordercolor = black}{}
%
%
%
%
%
%%===============================================================================================================
%%============================================  Gantt diagrams  =================================================
%%% GanttHeader setups some parameters for the rest of the diagram
%%% #1 Width of the diagram
%%% #2 Width of the space reserved for task numbers
%%% #3 Width of the space reserved for task names
%%% #4 Number of months in the diagram
%%% In addition to these parameters, the layout of the diagram is influenced
%%% by keys defined below, such as y, which changes the vertical scale
%%\def\GanttHeader#1#2#3#4{%
%%    \pgfmathparse{(#1-#2-#3)/#4}
%%    \tikzset{y=7mm, task number/.style={left, font=\bfseries},
%%        task description/.style={text width=#3,  right, draw=none,
%%            font=, xshift=#2,
%%            minimum height=2em},
%%        gantt bar/.style={draw=black, fill=blue!30},
%%        help lines/.style={draw=black!30, dashed},
%%        x=\pgfmathresult pt
%%    }
%%    \def\totalmonths{#4}
%%    \node (Header) [task description] at (0,0) {\textbf{\large Task Description}};
%%    \begin{scope}[shift=($(Header.south east)$)]
%%        \foreach \x in {1,...,#4}
%%        \node[above] at (\x,0) {\footnotesize\x};
%%    \end{scope}
%%}
%%
%%% This macro adds a task to the diagram
%%% #1 Number of the task
%%% #2 Task's name
%%% #3 Starting date of the task (month's number, can be non-integer)
%%% #4 Task's duration in months (can be non-integer)
%%\def\Task#1#2#3#4#5{%
%%    \node[task number] at ($(Header.west) + (0, -#1)$) {#5};
%%    \node[task description] at (0,-#1) {#2};
%%    \begin{scope}[shift=($(Header.south east)$)]
%%        \draw (0,-#1) rectangle +(\totalmonths, 1);
%%        \foreach \x in {1,...,\totalmonths}
%%        \draw[help lines] (\x,-#1) -- +(0,1);
%%        \filldraw[gantt bar] ($(#3, -#1+0.2)$) rectangle +(#4,0.6);
%%    \end{scope}
%%}
%
%
%
%
%% FIXME \renewcommand{\baselinestretch}{0.925}


==> Selective Sampling and Mixture Models in Generative Adversarial Networks/scratch.tex <==
bypassing the need for a domain-specific loss/cost function\\
GANs group close and similar representations together in the latent space\\



Improved GANs:\\
instance noise \cite{Casper ... 2016}\\
label noise \cite{Salimans_2016_ImprovedGAN}\\
one-sided label smoothing \cite{Salimans_2016_ImprovedGAN}\\




Graphical model view\\
Synthetic sample drawn from the generator\\
Minimize the mutual information between the two densities\\
Density function suffer from a non-overlapping support\\



























A generator network: $\hat{\bm{x}}^{(i)} = g_i(\bm{z})$\\
A generator network: $g_i(\bm{z};\,\bm{\theta}_{g_i})$\\
A generator network: $g_i: \bm{z} \rightarrow \bm{x}$\\
A discriminator network: $f_j(\bm{x})$\\
A discriminator network: $f_j(\bm{x}\,\bm{\theta}_{f_j})$\\
A discriminator network: $f_j: \bm{x}\rightarrow y$\\
Layers of G: $g_i: g_i^{(k_i)}\left(g_i^{(k_i-1)}\left( \dots \left(g_i^{(1)}(\bm{x})  \right)\right)\right)$\\
Layers of D: $f_j: f_j^{(l_j)}\left(f_j^{(l_j-1)}\left( \dots \left(f_j^{(1)}(\bm{x})  \right)\right)\right)$\\
Generator's cost function (i, j): $L_{g_i}(\bm{\theta}_{g_i}, \bm{\theta}_{f_j})$\\
Discriminator's cost function (i, j): $L_{f_j}(\bm{\theta}_{g_i}, \bm{\theta}_{f_j})$\\
Feature matching objective: \\$\norm{\mathbb{E}_{\bm{x}\sim p_{\text{data}}(\bm{x})}f_j^{(l)}(\bm{x}) -  \mathbb{E}_{\bm{z}_i\sim p_{\bm{z}_i}(\bm{z}_i)}f_j^{(l)}(g_i(\bm{z}_i)) }$\\
Real data distribution: $p_\text{data}(\bm{x})$\\
Generators' distribution: $p_{g_i}$\\





\small
\begin{align*}
\mathcal{L}_\text{cGAN}(G, D) = \;
	& \mathbb{E}_{\mathbf{x}, \mathbf{y}\sim p_{\text{data}}(\mathbf{x}, \mathbf{y})}\left[\log{D(\mathbf{x}, \mathbf{y})} \right] \plus \\
	& \mathbb{E}_{\mathbf{y}\sim p_{\text{data}}(\mathbf{y}),\, \mathbf{z}\sim p_\mathbf{z}(\mathbf{z})}\left[\log (1 - D(G(\mathbf{z}, \mathbf{y}), \mathbf{y})) \right]
\end{align*}
\normalsize
\small
\begin{align*}
\mathcal{L}_\text{L1}(G) = \;
	& \mathbb{E}_{\mathbf{x}, \mathbf{y}\sim p_{\text{data}}(\mathbf{x}, \mathbf{y}),\, \mathbf{z}\sim p_\mathbf{z}(\mathbf{z})}\left[ \norm{\mathbf{x} - G(\mathbf{z}, \mathbf{y})}_1 \right]
\end{align*}
\normalsize
\small

A minimax value function:
\begin{align*}
G^* = & \arg \min_G\max_D \left( \mathcal{L}_\text{cGAN}(G, D) + \lambda\,\mathcal{L}_\text{L1}(G) \right) \\
D^* = & \arg \min_D \left( \mathcal{L}_\text{cGAN}(G, D) \right)
\end{align*}
\normalsize

a batch $\{\mathbf{x}_i,\, \mathbf{y}_i\}_{i = 1}^n$ of training images $\mathbf{x}_i$ paired with conditional data $\mathbf{y}_i$


\textbf{EBGAN}:
\small
\begin{align*}
\mathcal{L}_D(\mathbf{x},\,\mathbf{z}) & =\, D(\mathbf{x}) + [m - D(G(\mathbf{z}))]^\plus  \\
\mathcal{L}_G(\mathbf{z}) 			   & =\, D(G(\mathbf{z})) \\
[\boldsymbol{\cdot}]                   & = max(0, \boldsymbol{\cdot})
\end{align*}
\normalsize



\color{DarkSlateGray4}




Image-to-Image Translation \cite{Isola_2016_Pix2Pix}



Conditional Generative Adversarial Networks (cGAN)

general-purpose solution to image-to-image translation

special-purpose machinery

loss formulation

In analogy to ...

... given sufficient training data

mapping is 

this problem is tackled with a special-purpose machinery.

CNN becoming the common workhorse behind a wide variety of ...

CNN + Euclidean Distance --> Blurry Results [Image2ImageTranslation[29, 46]]

all plausible outputs

a high-level goal

learn a loss function

GANs learn a loss that adapt to the data

GANs can be applied to a multitude of tasks that traditionally would require very different kinds of loss functions

GANs in the conditional setting

GANs have been vigorously studied in the last two years

Structured losses for image modeling

per-pixel classification/regression formulation treat the output space as 'unstructured' in the sense that ...

cGANs learn a structured loss ... (the joint configuration is awarded or penalized on a whole object basis not on a per-pixel basis)


[Very Important]
Structured losses: 
	1) Conditional Random Fields [Chen 2015 ... Semantic Image SEgmentation with Deep Convolutional Nets and Fully Connected CRFs]
	2) SSIM Metric [Wang 2004 ... Image Quality Assessment from error Visibility to structural Similarity]
	3) Feature matching [Dosovitskiy 2016 ... Generating images with perceptual similarity metrics based on deep networks]
	4) Non-Parametric loss [Li 2016 .. Combining Markov RAndom Fields and Convolutional Neural Networks for Image Synthesis]
	5) Convolutional Pseudo-Prior [Xie 2015 ... Top-Down learning for Structured Labeling with Convolutional Pseudo-Prior]
	6) Matching Covariance Statistics [Johnson 2016 ... Perceptual Losses for real-time style transfer and super-resolution]
	

Adversarially trained discriminator

this is diagrammed in figure ...

shuttle

prominent edges

a means to circumvent the bottleneck 

high frequency crispness

L1 and L2 losses fail to encourage high frequency crispness but in many cases they accurately capture the low frequencies


advantageous


PatchGAN --> texture/style loss

qualitative results

traditional metrics such as MSE do not asses joint statistics of the result 

holistically evaluate the visual quality

we employ two tactics

perceptual study

plausibility to a human observer is the ultimate goal

vigilance trial

aerial photo

floor-level results

discriminability

as a Pseudo Metric

ablation studies

L1 will incentivize a blur

L1 will be minimized by choosing the median of the conditional probability density function over possible colors

adversarial loss

PixelGAN vs PatchGAN vs ImageGAN

tiling artifacts


a factored generative network style






RBMs and many variants have been used in confined settings

development has been stunted

SGD training regime

sidestep (v.) 

The generative model yielded by a learned GAN can serve as a density model of the training data

using incorporated conditional data as priors on generation

poses the two players in an adversarial game


For the moment, we explain the two terms of the equation in prose:

adding a conditioning ability to the GAN framework

$Z = \mathbb{R}^{d_Z}$ is a noise space used to seed the generative model and $d_z$ is its dimensionality and it is a hyperparameter. Values $\mathbf{z} \in Z$ are sampled from the noise distribution $p_\mathbf{z}(\mathbf{z})$.

$Y = \mathbb{R}^{d_Y}$ is an embedding space used to condition the generative model on some external information drawn from the training data.

empirical data distribution vs generative model

The discriminator becomes more attuned to real features in order to distinguish between the simple images from the generator and real ones.

This process continues ad infinitum .... until the discriminator is maximally confused ... which is expected when the discriminator consistently output a probability of 0.5 for inputs form either real data or generated images.

The discriminator loss trends toward a theoretically maximal confusion

Model Architecture


evidently helps to prevent overfitting the training data


 
















EBGAN exhibits more stable behavior than regular GANs during training

A single-scale architecture (of EBGAN) can be trained to generate high-resolution images.

lower energy is attributed to the data manifold 

The generator uses input from an easy-to-sample random source

From a game theory point of view, the convergence of a GAN is reached when the generator and the discriminator reach a Nash equilibrium.

Discriminator --> Energy function / Contrast function

The energy function computed by the discriminator can be viewed as a trainable cost function for the generator.

Probabilistic GAN

at the first glance

we postulate that an auto-encoder architecture for the discriminator is conceptually more attractive than a binary logistic network

in EBGAN the discriminator (i.e. the energy function or the auto-encoder) is being regularized by having a generator that continuously produces contrastive samples to which the discriminator ought to assign high energy values.

The regularizer in EBGAN (i.e. the generator) is parametric and fully trainable rather than handcrafted.

... purposely doing ...

Repelling regularization vs Mini-batch discrimination

primarily

the work casts GANs into an energy-based model scope




















Source vs Target domain

Semantic meaning

overcoming the semantic gap between the two domains




One-sided label smoothing

Two-sided label smoothing

Penalizing confident decisions/predictions

Virtual Batch Normalization












{\noindent\color{Maroon3}
Finite Mixture Model\\
Sampling from a population that consists of several homogeneous subpopulations or components.\\
Component densities\\
Component parameter\\
Component weight $\pi_j$: The proportion of the total population in the $j^{\text{th}}$ component.\\
$\sum_j \pi_j = 1$ \\
Joint density:\\ {\scriptsize $Pr(X = x, J = j) = Pr(X = x | J = j) \cdot Pr(J = j) = p(x; \zeta_j) \dots \pi_j$}\\
The mixture model arises if the component label data $J_1, \cdots, J_n$ is missing so that we observe only the samples $X_1, \dots, X_n$ from the marginal density of $X$. \\
Mixture density:\\ {\small $ g(x; \pi, \Theta) = \sum P(X = x| J= j) P(J = j) = \sum \pi_j \cdot f(x\;\zeta_j)$}\\
MultiGAN address the a finite mixture model of $m$ non-homogeneous component densities. \\
A mixture of $m$ non-homogeneous components \\
Relatively homogeneous components\\
Mixture analysis \\
surrogate measure vs ideal measure\\
}


{\noindent\color{LightYellow4}

}











synthetic images\\
under mild conditions\\




multi-scale structure of natural images\\
plausible looking scenes\\
a cascade / series of generative models \\
Laplacian pyramid\\
breaks the problem into a sequence of more manageable stages\\
coarse-to-fine fashion\\
commencing with (beginning with)\\
band-pass structure \\
straightforward to train and sample from\\
with the resulting samples showing a surprising level of visual fidelity\\
stochastically chosen sample\\

the well-known problem of mode collapse\\



{\color{red}
	DCGAN\\
	approximate generalization performance by cross validation\\
	leverage the practically unlimited amount of unlabeled data\\
	learn good intermediate representations\\
	a variety of supervised learning tasks\\
	feature extractors for supervised tasks\\
	GANs provide an attractive alternative to ML techniques\\
	lack of heuristic cost function\\
	generators that produce nonsensical outputs\\
	architectural topology of GANs\\
	leverage clusters for improved classification scores\\
	images looking wobbly\\
	replacing deterministic spatial pooling functions (max-pool) with strided convolutions: all conv. net\\
	trend towards eliminating fully connected layers\\
	convolution stack\\
	a common failure mode observed in GANs\\
	sample oscillation and model instability\\
	memorization of training samples\\
	semantically relevant\\
	
}



==> chapters/introduction-and-related-work.tex <==
\section{Introduction and Related Work}
\label{sec:introduction-and-related-work}

One of the popular unsupervised learning methods is generative modeling, and in the recent years a promising architecture, referred to as \ul{G}enerative \ul{A}dversarial \ul{N}etworks (GAN) \cite{Goodfellow_2014_GAN}, has attracted a wide interest due to their impressive success in various applications domains, including text-to-image generation \cite{Reed_2016_Text2Image}, image-to-image translation \cite{Isola_2016_Pix2Pix}, multi- and super-resolution image synthesis \cite{Denton_2015_LaplacianPyramids}, video generation \cite{Vondrick_2016_GeneratingVideos}, in addition to a variety of  unsupervised and semi-supervised learning tasks \cite{Shrivastava_2016_SimulatedGANApple, Springenberg_2015_CatGAN, Zhu_2017_CycleConsistentGAN}. The common principle behind all variants of the GAN architecture is to exploit the discriminative power of neural networks in training generative counterparts. GAN models represent a compromise between ease of sampling and perceptual quality of synthesized samples.


Similar to other generative models, the ultimate objective of GANs is to model a target distribution from a limited set of observations.


% In addition, GANs feature ease of sampling with high perceptual quality \cite{}. 
% A generative network is tasked with estimating a real data distribution, while a discriminative one is tasked with training the former how to achieve their task. The generator does not explicitly model the real data distribution; instead, it learns how to synthesize data samples that are almost indistinguishable from the real ones.
% GANs resemble a compromise between ease of sampling and perceptual quality. When compared to Maximum Likelihood (ML) models, the latter tend to over-generalize the target distribution at the expense of perceptual quality \cite{Theis_2015_GANEvaluation}.

==> figures/cnn_net.tex <==
%draw a cnn layer with input and output feature maps and with kernels
\scalebox{0.5}{
\begin{tikzpicture}
    \definecolor{myblue}{cmyk}{1,0,0,0}
    \definecolor{myred}{cmyk}{0,1,0,0}
    \node[] at (0.5,5.5,0) {\Large \bf The convolutional layer};
    
    %draw input feature map
    \draw[white](0,0,0)--(0,4,0)--(1,4,0)--(1,0,0)--(0,0,0);
    \draw[white](1,0,0)--node[color=black,right]{$M$}(1,0,4)--(1,4,4)--(1,4,0)--(1,0,0);
    \draw[white](1,0,4)--node[color=black,below]{$O$}(0,0,4)--(0,4,4)--(1,4,4)--(1,0,4);
    \draw[white](0,0,4)--(0,0,0)--(0,4,0)--(0,4,4)--node[color=black,left]{$N$}(0,0,4);
    %caption
    \node[] at (0.5,4.5,0) {Input $\X$};
                
    %draw first kernel
    \draw[white](3.5,0.5,1.5)--(3.5,1.5,1.5)--(4.5,1.5,1.5)--(4.5,0.5,1.5)--(3.5,0.5,1.5);
    \draw[white](4.5,0.5,1.5)--(4.5,0.5,2.5)--(4.5,1.5,2.5)--(4.5,1.5,1.5)--(4.5,0.5,1.5);
    \draw[white](4.5,0.5,2.5)--(3.5,0.5,2.5)--(3.5,1.5,2.5)--(4.5,1.5,2.5)--(4.5,0.5,2.5);
    \draw[white](3.5,0.5,2.5)--(3.5,0.5,1.5)--(3.5,1.5,1.5)--(3.5,1.5,2.5)--(3.5,0.5,2.5);
    
    %draw dots inbetween
    \draw[dashed](3.5,1.5,1.5)--(3.5,2.5,1.5);
    \draw[dashed](4.5,1.5,1.5)--(4.5,2.5,1.5);
    \draw[dashed](4.5,1.5,2.5)--(4.5,2.5,2.5);
    \draw[dashed](3.5,1.5,2.5)--(3.5,2.5,2.5);
    
    %draw second kernel
    \draw[white](3.5,2.5,1.5)--(3.5,3.5,1.5)--(4.5,3.5,1.5)--(4.5,2.5,1.5)--(3.5,2.5,1.5);
    \draw[white](4.5,2.5,1.5)--(4.5,2.5,2.5)--(4.5,3.5,2.5)--(4.5,3.5,1.5)--(4.5,2.5,1.5);
    \draw[white](4.5,2.5,2.5)--node[color=black,below]{$\:\:O$}(3.5,2.5,2.5)--(3.5,3.5,2.5)--(4.5,3.5,2.5)--(4.5,2.5,2.5);
    \draw[white](3.5,2.5,2.5)--(3.5,2.5,1.5)--(3.5,3.5,1.5)--node[color=black,left]{$K$}(3.5,3.5,2.5)--node[color=black,left]{$K$}(3.5,2.5,2.5);
    %caption
    \node[] at (3.5,3.5,0) {Kernel tensor $\W$};
    
    %draw input feature maps
    \foreach \x in {0,0.25,0.5,0.75,1}{    
        \pgfmathsetmacro\k{(\x+0.1)*50}
            \draw[black, fill=black!\k](\x,0,4)--(\x,0,0)--(\x,4,0)--(\x,4,4)--(\x,0,4);}
    
    %draw selected region for convolution
    \draw[black](1,2,3)--(1,2,2)--node[color=black,right]{$\X(m,n)$}(1,3,2)--(1,3,3)--(1,2,3);
    
    %draw connections to kernels
    \draw[dashed](1,2,3)--(3.5,0.5,2.5);
    \draw[dashed](1,3,3)--(3.5,3.5,2.5);
    \draw[dashed](1,2,2)--(3.5,0.5,1.5);
    \draw[dashed](1,3,2)--(3.5,3.5,1.5);
    
    %draw first kernel
    \foreach \x in {0,0.25,0.5,0.75,1}{    
        \pgfmathsetmacro\k{(\x+0.1)*100}
        \draw[black, fill=myblue!\k](3.5+\x,0.5,2.5)--(3.5+\x,0.5,1.5)--(3.5+\x,1.5,1.5)--(3.5+\x,1.5,2.5)--(3.5+\x,0.5,2.5);}

    %draw second kernel
    \foreach \x in {0,0.25,0.5,0.75,1}{    
        \pgfmathsetmacro\k{(\x+0.1)*100}
        \draw[black, fill=myred!\k](3.5+\x,2.5,2.5)--(3.5+\x,2.5,1.5)--(3.5+\x,3.5,1.5)--(3.5+\x,3.5,2.5)--(3.5+\x,2.5,2.5);}
    
    %draw output feature map with convolution results
    \draw[black](7,0,0)--(7,4,0)--(8,4,0)--(8,0,0)--(7,0,0);
    \draw[black](8,0,0)--node[color=black,right]{$M-K+1$}(8,0,4)--(8,4,4)--(8,4,0)--(8,0,0);
    \draw[black](7,0,4)--(7,0,0)--(7,4,0)--(7,4,4)--node[right]{$N-K+1$}(7,0,4);
    
    \foreach \x in {0,0.25,0.5,0.75,1}{    
        \pgfmathsetmacro\k{(\x+0.1)*50}
        (1,2,3)--(1,2,2)--(1,3,2)--(1,3,3)--(1,2,3)
            \draw[black, fill=black!\k](\x+7,2.25,2.75)--(\x+7,2.25,2.25)--(\x+7,2.75,2.25)--(\x+7,2.75,2.75)--(\x+7,2.25,2.75);}
            
    \draw[black](8,0,4)--node[below]{$P$}(7,0,4)--(7,4,4)--(8,4,4)--(8,0,4);
    
    %draw connections to kernels
    
    \draw[dashed](4.5,3.5,2.5)--(7,2.75,2.75);
    \draw[dashed](4.5,0.5,1.5)--(7,2.25,2.25);
    \draw[dashed](4.5,3.5,1.5)--(7,2.75,2.25);
    
    %draw bias
    \foreach \y in {1,2,3,4,5}{    
        \pgfmathsetmacro\k{((\y-1)/4+0.1)*50}
            \fill [black!\k] (5 ,1-\y*0.5,2) rectangle (5.5,1.5-\y*0.5,2);}
    
    \draw[dashed](4.5,0.5,2.5)--(7,2.25,2.75);
    
    
    %caption
    \node[] at (7.5,4.5,0) {Activation $\A$};  
    \node[] at (4.5,-2.5,0) {Bias $\bi$};  
    
    %operators
    \node[] at (2.5,2,2) {$*$}; 
    \node[] at (5.25,2,2) {$+$};
    \node[] at (6.25,2,2) {$=$}; 
    
    %kernel index
    \node[] at (4,3,2) {$1$};
    \node[] at (4,1,2) {$P$}; 
    
    \draw[dashed](9.5,5,0)--(9.5,-2,0);
    \node[] at (9.5,-2.25,0) {unfolding};
    

    %draw unfolded 
    \node[] at (2.0+11-0.75,5.5,0) {\Large \bf The equivalent dense layer};
    \definecolor{myblue}{cmyk}{1,0,0,0}
    \definecolor{myred}{cmyk}{0,1,0,0}

    %captions
    \node[] at (1.5+10-0.75,5-0.5,0) {Activation $\ai$};
    \node[] at (1.5+10+3,5-0.5,0) {Kernel matrix $\Wu$};
    \node[] at (1.5+10+8,5-0.5,0) {Input $\x$};
    \node[] at (1.5+10+9.75,5-0.5,0) {Bias $\bi$};
    
    %operators
    \node[] at (1.5+10+0.5,2.75-0.5,0) {$=$};
    \node[] at (1.5+10+7.5,2.75-0.5,0) {$\cdot$};
    \node[] at (1.5+10+9.0,2.75-0.5,0) {$+$};
    
    %The unfolded matrix
    \foreach \x in {1,2,3,4,5}{
        \foreach \y in {1,2,3,4,5}{
            \pgfmathsetmacro\c{1.0-(\y-1)*0.25}
            \pgfmathsetmacro\m{(\y-1)*0.25}
            \definecolor{mix}{cmyk}{\c,\m,0,0}
            \pgfmathsetmacro\k{((\x-1)/5+0.1)*100}
            \fill [mix!\k] (1.5+10+2+\x*1,\y*0.5+1.5-0.5,0) rectangle (1.5+10+2+\x*1-1,\y*0.5-0.5+1.5-0.5,0);
         }
    }
    
    %draw unfolded input feature map
    \foreach \y in {1,2,3,4,5}{    
        \pgfmathsetmacro\k{((\y-1)/4+0.1)*50}
            \fill [black!\k] (1.5+10+8,4-\y-0.5,0) rectangle (1.5+10+8.5,4-\y+1-0.5,0);}
    
    %draw unfolded output feature map
    \foreach \y in {1,2,3,4,5}{    
        \pgfmathsetmacro\k{((\y-1)/4+0.1)*50}
            \fill [black!\k] (1.5+10-1,4-\y*0.5-0.5,0) rectangle (1.5+10-0.5,4.5-\y*0.5-0.5,0);}
    
    %draw bias
    \foreach \y in {1,2,3,4,5}{    
        \pgfmathsetmacro\k{((\y-1)/4+0.1)*50}
            \fill [black!\k] (1.5+10+9.5,4-\y*0.5-0.5,0) rectangle (1.5+10+10,4.5-\y*0.5-0.5,0);}
    
    %give the size of the unfolded matrix
    \node[] at (1.5+10+1.8,2.75-0.5,0) {$P$};
    \node[] at (1.5+8.8,2.75-0.5,0) {$P$};
    \node[] at (1.75+20,2.75-0.5,0) {$P$};
    \node[] at (1.5+10+4.5,4.2-0.5,0) {$K^2O$};
    \node[] at (1.5+10+9,1.5-0.5,0) {$K^2O$};
\end{tikzpicture}}


==> literature.tex <==
List of references:
   
   
... PRINTED
1. Generative Image Modeling using Style and Structure Adversarial Networks ... Wang 2016
2. Generative Adversarial Nets ... Goofellow 2014
3. Deep Generative Image Models using a Laplacian Pyramid of Adversarial Networks ... Denton 2015
4. On distinguishability criteria for estimating generative models ... Goodfellow 2015
1. Energy-Based GAN (EBGAN) ... Zhao 2017
1. Deep Directed Generative Models with Energy-Based Probability Estimation ... Kim 2016
1. Unsupervised Representation Learning with Deep Convolutional Generative Adversarial Networks ... Radford 2015
1. Pixel-level domain transfer ... Yoo 2016
1. Unsupervised and Semi-Supervised Learning with Categorical Generative Adversarial Networks ... Springenberg 2015
1. Conditional Generative Adversarial Nets for Convolutional Face Generation ... Gauthier 2015
1. Conditional Generative Adversarial Nets ... Mirza 2014
1. Deep Multi-Scale Video Prediction Beyond Mean Square Error ... Mathieu 2015
1. Generating Images with Recurrent Adversarial Networks ... Im 2016
1. Adversarial Auto Encoders ... Machzani 2015
1. Auto-encoding beyond pixels using a learned Similarity Metric ... Larsen 2015
1. Generating Images with Perceptual Similarity Metrics based on Deep Networks ... Dosovitskiy 2016
1. Improved Techniques for Training GANs ... Salimans 2016
1. Generative Visual Manipulation on the Natural Image Manifold ... Zhu 2016
1. Context Encoder: Feature Learning by Inpainting ... Pathak 2016
1. Generating Video with Scene Dynamics ... Vondrick 2016
1. Learning a Probabilistic Latent Space of Object Shapes vis 3D Generative Adversarial Modeling ... Wu 2016

... UNSURE


==> scratch.tex <==
bypassing the need for a domain-specific loss/cost function\\
GANs group close and similar representations together in the latent space\\



Improved GANs:\\
instance noise \cite{Casper ... 2016}\\
label noise \cite{Salimans_2016_ImprovedGAN}\\
one-sided label smoothing \cite{Salimans_2016_ImprovedGAN}\\




Graphical model view\\
Synthetic sample drawn from the generator\\
Minimize the mutual information between the two densities\\
Density function suffer from a non-overlapping support\\



























A generator network: $\hat{\bm{x}}^{(i)} = g_i(\bm{z})$\\
A generator network: $g_i(\bm{z};\,\bm{\theta}_{g_i})$\\
A generator network: $g_i: \bm{z} \rightarrow \bm{x}$\\
A discriminator network: $f_j(\bm{x})$\\
A discriminator network: $f_j(\bm{x}\,\bm{\theta}_{f_j})$\\
A discriminator network: $f_j: \bm{x}\rightarrow y$\\
Layers of G: $g_i: g_i^{(k_i)}\left(g_i^{(k_i-1)}\left( \dots \left(g_i^{(1)}(\bm{x})  \right)\right)\right)$\\
Layers of D: $f_j: f_j^{(l_j)}\left(f_j^{(l_j-1)}\left( \dots \left(f_j^{(1)}(\bm{x})  \right)\right)\right)$\\
Generator's cost function (i, j): $L_{g_i}(\bm{\theta}_{g_i}, \bm{\theta}_{f_j})$\\
Discriminator's cost function (i, j): $L_{f_j}(\bm{\theta}_{g_i}, \bm{\theta}_{f_j})$\\
Feature matching objective: \\$\norm{\mathbb{E}_{\bm{x}\sim p_{\text{data}}(\bm{x})}f_j^{(l)}(\bm{x}) -  \mathbb{E}_{\bm{z}_i\sim p_{\bm{z}_i}(\bm{z}_i)}f_j^{(l)}(g_i(\bm{z}_i)) }$\\
Real data distribution: $p_\text{data}(\bm{x})$\\
Generators' distribution: $p_{g_i}$\\





\small
\begin{align*}
\mathcal{L}_\text{cGAN}(G, D) = \;
	& \mathbb{E}_{\mathbf{x}, \mathbf{y}\sim p_{\text{data}}(\mathbf{x}, \mathbf{y})}\left[\log{D(\mathbf{x}, \mathbf{y})} \right] \plus \\
	& \mathbb{E}_{\mathbf{y}\sim p_{\text{data}}(\mathbf{y}),\, \mathbf{z}\sim p_\mathbf{z}(\mathbf{z})}\left[\log (1 - D(G(\mathbf{z}, \mathbf{y}), \mathbf{y})) \right]
\end{align*}
\normalsize
\small
\begin{align*}
\mathcal{L}_\text{L1}(G) = \;
	& \mathbb{E}_{\mathbf{x}, \mathbf{y}\sim p_{\text{data}}(\mathbf{x}, \mathbf{y}),\, \mathbf{z}\sim p_\mathbf{z}(\mathbf{z})}\left[ \norm{\mathbf{x} - G(\mathbf{z}, \mathbf{y})}_1 \right]
\end{align*}
\normalsize
\small

A minimax value function:
\begin{align*}
G^* = & \arg \min_G\max_D \left( \mathcal{L}_\text{cGAN}(G, D) + \lambda\,\mathcal{L}_\text{L1}(G) \right) \\
D^* = & \arg \min_D \left( \mathcal{L}_\text{cGAN}(G, D) \right)
\end{align*}
\normalsize

a batch $\{\mathbf{x}_i,\, \mathbf{y}_i\}_{i = 1}^n$ of training images $\mathbf{x}_i$ paired with conditional data $\mathbf{y}_i$


\textbf{EBGAN}:
\small
\begin{align*}
\mathcal{L}_D(\mathbf{x},\,\mathbf{z}) & =\, D(\mathbf{x}) + [m - D(G(\mathbf{z}))]^\plus  \\
\mathcal{L}_G(\mathbf{z}) 			   & =\, D(G(\mathbf{z})) \\
[\boldsymbol{\cdot}]                   & = max(0, \boldsymbol{\cdot})
\end{align*}
\normalsize



\color{DarkSlateGray4}




Image-to-Image Translation \cite{Isola_2016_Pix2Pix}



Conditional Generative Adversarial Networks (cGAN)

general-purpose solution to image-to-image translation

special-purpose machinery

loss formulation

In analogy to ...

... given sufficient training data

mapping is 

this problem is tackled with a special-purpose machinery.

CNN becoming the common workhorse behind a wide variety of ...

CNN + Euclidean Distance --> Blurry Results [Image2ImageTranslation[29, 46]]

all plausible outputs

a high-level goal

learn a loss function

GANs learn a loss that adapt to the data

GANs can be applied to a multitude of tasks that traditionally would require very different kinds of loss functions

GANs in the conditional setting

GANs have been vigorously studied in the last two years

Structured losses for image modeling

per-pixel classification/regression formulation treat the output space as 'unstructured' in the sense that ...

cGANs learn a structured loss ... (the joint configuration is awarded or penalized on a whole object basis not on a per-pixel basis)


[Very Important]
Structured losses: 
	1) Conditional Random Fields [Chen 2015 ... Semantic Image SEgmentation with Deep Convolutional Nets and Fully Connected CRFs]
	2) SSIM Metric [Wang 2004 ... Image Quality Assessment from error Visibility to structural Similarity]
	3) Feature matching [Dosovitskiy 2016 ... Generating images with perceptual similarity metrics based on deep networks]
	4) Non-Parametric loss [Li 2016 .. Combining Markov RAndom Fields and Convolutional Neural Networks for Image Synthesis]
	5) Convolutional Pseudo-Prior [Xie 2015 ... Top-Down learning for Structured Labeling with Convolutional Pseudo-Prior]
	6) Matching Covariance Statistics [Johnson 2016 ... Perceptual Losses for real-time style transfer and super-resolution]
	

Adversarially trained discriminator

this is diagrammed in figure ...

shuttle

prominent edges

a means to circumvent the bottleneck 

high frequency crispness

L1 and L2 losses fail to encourage high frequency crispness but in many cases they accurately capture the low frequencies


advantageous


PatchGAN --> texture/style loss

qualitative results

traditional metrics such as MSE do not asses joint statistics of the result 

holistically evaluate the visual quality

we employ two tactics

perceptual study

plausibility to a human observer is the ultimate goal

vigilance trial

aerial photo

floor-level results

discriminability

as a Pseudo Metric

ablation studies

L1 will incentivize a blur

L1 will be minimized by choosing the median of the conditional probability density function over possible colors

adversarial loss

PixelGAN vs PatchGAN vs ImageGAN

tiling artifacts


a factored generative network style






RBMs and many variants have been used in confined settings

development has been stunted

SGD training regime

sidestep (v.) 

The generative model yielded by a learned GAN can serve as a density model of the training data

using incorporated conditional data as priors on generation

poses the two players in an adversarial game


For the moment, we explain the two terms of the equation in prose:

adding a conditioning ability to the GAN framework

$Z = \mathbb{R}^{d_Z}$ is a noise space used to seed the generative model and $d_z$ is its dimensionality and it is a hyperparameter. Values $\mathbf{z} \in Z$ are sampled from the noise distribution $p_\mathbf{z}(\mathbf{z})$.

$Y = \mathbb{R}^{d_Y}$ is an embedding space used to condition the generative model on some external information drawn from the training data.

empirical data distribution vs generative model

The discriminator becomes more attuned to real features in order to distinguish between the simple images from the generator and real ones.

This process continues ad infinitum .... until the discriminator is maximally confused ... which is expected when the discriminator consistently output a probability of 0.5 for inputs form either real data or generated images.

The discriminator loss trends toward a theoretically maximal confusion

Model Architecture


evidently helps to prevent overfitting the training data


 
















EBGAN exhibits more stable behavior than regular GANs during training

A single-scale architecture (of EBGAN) can be trained to generate high-resolution images.

lower energy is attributed to the data manifold 

The generator uses input from an easy-to-sample random source

From a game theory point of view, the convergence of a GAN is reached when the generator and the discriminator reach a Nash equilibrium.

Discriminator --> Energy function / Contrast function

The energy function computed by the discriminator can be viewed as a trainable cost function for the generator.

Probabilistic GAN

at the first glance

we postulate that an auto-encoder architecture for the discriminator is conceptually more attractive than a binary logistic network

in EBGAN the discriminator (i.e. the energy function or the auto-encoder) is being regularized by having a generator that continuously produces contrastive samples to which the discriminator ought to assign high energy values.

The regularizer in EBGAN (i.e. the generator) is parametric and fully trainable rather than handcrafted.

... purposely doing ...

Repelling regularization vs Mini-batch discrimination

primarily

the work casts GANs into an energy-based model scope




















Source vs Target domain

Semantic meaning

overcoming the semantic gap between the two domains




One-sided label smoothing

Two-sided label smoothing

Penalizing confident decisions/predictions

Virtual Batch Normalization












{\noindent\color{Maroon3}
Finite Mixture Model\\
Sampling from a population that consists of several homogeneous subpopulations or components.\\
Component densities\\
Component parameter\\
Component weight $\pi_j$: The proportion of the total population in the $j^{\text{th}}$ component.\\
$\sum_j \pi_j = 1$ \\
Joint density:\\ {\scriptsize $Pr(X = x, J = j) = Pr(X = x | J = j) \cdot Pr(J = j) = p(x; \zeta_j) \dots \pi_j$}\\
The mixture model arises if the component label data $J_1, \cdots, J_n$ is missing so that we observe only the samples $X_1, \dots, X_n$ from the marginal density of $X$. \\
Mixture density:\\ {\small $ g(x; \pi, \Theta) = \sum P(X = x| J= j) P(J = j) = \sum \pi_j \cdot f(x\;\zeta_j)$}\\
MultiGAN address the a finite mixture model of $m$ non-homogeneous component densities. \\
A mixture of $m$ non-homogeneous components \\
Relatively homogeneous components\\
Mixture analysis \\
surrogate measure vs ideal measure\\
}


{\noindent\color{LightYellow4}

}











synthetic images\\
under mild conditions\\




multi-scale structure of natural images\\
plausible looking scenes\\
a cascade / series of generative models \\
Laplacian pyramid\\
breaks the problem into a sequence of more manageable stages\\
coarse-to-fine fashion\\
commencing with (beginning with)\\
band-pass structure \\
straightforward to train and sample from\\
with the resulting samples showing a surprising level of visual fidelity\\
stochastically chosen sample\\

the well-known problem of mode collapse\\



{\color{red}
	DCGAN\\
	approximate generalization performance by cross validation\\
	leverage the practically unlimited amount of unlabeled data\\
	learn good intermediate representations\\
	a variety of supervised learning tasks\\
	feature extractors for supervised tasks\\
	GANs provide an attractive alternative to ML techniques\\
	lack of heuristic cost function\\
	generators that produce nonsensical outputs\\
	architectural topology of GANs\\
	leverage clusters for improved classification scores\\
	images looking wobbly\\
	replacing deterministic spatial pooling functions (max-pool) with strided convolutions: all conv. net\\
	trend towards eliminating fully connected layers\\
	convolution stack\\
	a common failure mode observed in GANs\\
	sample oscillation and model instability\\
	memorization of training samples\\
	semantically relevant\\
	
}


